Interim Report on Human-Guided Adaptive Hyperparameter Optimization with Multi-Fidelity Sprints

This case study applies a phased hyperparameter optimization process to compare multitask natural language model variants that utilize multiphase learning rate scheduling and optimizer parameter grouping. We employ short, Bayesian optimization sessions that leverage multi-fidelity, hyperparameter space pruning, progressive halving, and a degree of human guidance. We utilize the Optuna TPE sampler and Hyperband pruner, as well as the Scikit-Learn Gaussian process minimization. Initially, we use efficient low-fidelity sprints to prune the hyperparameter space. Subsequent sprints progressively increase their model fidelity and employ hyperband pruning for efficiency. A second aspect of our approach is using a meta-learner to tune threshold values to resolve classification probabilities during inference. We demonstrate our method on a collection of variants of the 2021 Joint Entity and Relation Extraction model proposed by Eberts and Ulges.

==> 03-Cascading-Project.tex <==
Given that this is a multi-faceted project, it may move in various directions.

\begin{itemize}
    \item It may result in one or more paper publications
    \item It may serve as a tutorial or educational resource
    \begin{itemize}
        \item Book with code
        \item Illustrate the application of relevant techniques and enhancements
        \item Demonstrate coding techniques
        \item Pytorch Lightning demonstration
        \item Torch 2.x feature demonstration, e.g. compilation
    \end{itemize}
    \item It may be refocused on a small number of enhancements and lead to a conference publication. 
    \item It may lead to open software contributions.
    \item Papers with Code 
    
\end{itemize}

==> 10A_Introduction.tex <==
This study examines ways to improve the performance of JEREX, a joint multitask multi-instance entity and relation extraction model \cite{eberts-ulges-2021-end}  trained and tested on DocRED \cite{yao-etal-2019-docred}. We named our modified version JEREX-L\footnote{The suffix ``-L" was conceived initially to denote the handling of longer passages by switching the shared encoder transformer from Bert to Longformer}. We assume the reader to be familiar with \href{https://arxiv.org/abs/2102.05980v2}{the original work} by \cite{eberts-ulges-2021-end}, so we avoid repetition and only focus on areas relevant to our study, which we summarize below:

\begin{description}
    \item[The Dataset:]
    What is challenging about DocRED is that it contains multi-sentence examples annotated for six named entity types and 96 relation classes, some of which require reasoning through multiple sentences to predict correctly. To circumvent a well-known issue with DocRed, i.e., its incomplete annotations, we train and test JEREX-L  on Re-DocRED \cite{tan2022revisiting}, which addresses many of these issues. 
    
    \item[Learning Rate Search:] 
    We partitioned the model's parameters into distinct groups: two for the shared transformer modules and one for each of the four task modules.  This increased the complexity of hyperparameter search and scheduling strategy determination, rendering manual grid-based methods impractical. Our challenge was to find a way to compare scores across different model configurations and options in a consistent and relatively efficient way. Bayesian techniques \cite{frazier2018tutorial} helped us improve consistency and relative efficiency. For implementation, we leverage the \href{https://scikit-optimize.github.io/stable/auto_examples/bayesian-optimization.html}{skopt} optimization core framework. %Additionally, we established a standardized protocol for deriving optimal learning rates for each configuration and set of options we tested.  
    
    \item[Threshold Meta-Learner:] Prediction performance is highly sensitive to the choice of three thresholds, which are typically determined via grid search. This process had to be repeated for each of the configurations we tested. We introduced a hill-climbing meta-learner and added a configurable calibration phase to the training-validation cycle to ensure consistency and effectiveness in threshold tuning. This meta-learner optimizes the thresholds to maximize the relation F1-micro score, streamlining their value selection. 
    
    Moreover, we implemented an analytical optimization algorithm, specific to mention thresholds, that maximizes the mention-F1-micro score at the end of each validation. 
    
    %Relation extraction inference in JEREX involves three interdependent multi-label classification tasks:  entity mention localization, coreference resolution, and relation classification. To convert classifier output to discrete predictions, the original model uses three scalar thresholds. 
    
    Since the relation classifier is multi-label and multi-class, we replaced the original single global scalar threshold with a vector of thresholds optimized independently and specific to each class.
    
    The strategy for running our experiments was empirically derived. 
    
    \item [Encoder Model:] The original JEREX model uses \emph{bert-base-cased} as the encoder. %, limiting the input sequence to 512 tokens, as most regular transformers. %This input size limitation of most standard transformer models is due to the quadratic cost of self-attention. 
    We generalized the framework to enable several auto-model transformers from Hugging Face \cite{wolf-etal-2020-transformers} through configurable arguments. Many of the results in this article use \emph{longformer-base-4096} \cite{Beltagy2020Longformer} by Allen AI, which allows longer input sequences and can accommodate all examples of the DocRED and re-DocRED datasets. 
    The Longformer architecture features a memory-efficient attention mechanism that can handle long passages at nearly linear cost. It combines local (windowed) and global attention, which resonate well with spoken or written language, where semantic word linkages tend to diminish with distance but occasional important exceptions exist and must be handled.
    %The Longformer architecture features a more memory-efficient attention mechanism, combining local (windowed) and global attention semantic word linkages in a language tends to diminish with distance, resonating with the concept of windowed (local) attention. Occasional exceptions, such as proper nouns, can be addressed by global attention. 
    \item[Linguistic Augmentation:] The main component of the original representation of mentions and relations consists of contextual embeddings generated by the encoder transformer. We hypothesize that adding linguistic features, such as part-of-speech (POS) or structural dependencies (DEP), may enhance performance. We employ \emph{Spacy} to do this. Encodings of these linguistic features extend the hidden representation for Bert and other encoders. Specifically for Longformer, we use nouns and proper nouns as the global attention features.
    \item[Representation Changes:] The representation of distances was changed from embeddings to log-linear transformations (\autoref{sec:RepChanges}). 
    \item[Data Imbalance] The original model controls the proliferation of negative examples by limiting their sampling to a fixed count and by favoring the more complex negative instances whose spans overlap with positive ones. We consider the following additional enhancements: (a) Controlling negative sample size based on a fixed negative-to-positive ratio instead of a fixed limit. (b) Enabling adaptive asymmetric loss as a function of prediction difficulty \cite{benbaruch2020asymmetric}. %This technique accentuates losses of negative samples that the model finds more challenging, i.e., less confident predictions, and deemphasizes losses of the less challenging ones, i.e., more confident ones. 
    Asymmetry pertains to parameterizing positive examples differently than negative ones. 
    \item[Multitask Learning (MTL) and Finetuning:] The JEREX multitask learning (MTL) architecture combines four classifier tasks that share the state of an encoder, originally implemented as a BERT transformer. The multitask loss calculation uses fixed weights to combine the four respective losses. We added instrumentation to examine the norm and cosine similarity of gradients coming from the component task models. We then considered various confidence-based weighting techniques to calculate better multitask loss or to manipulate the gradients directly. 
    
    To visualize how conflicting adaptations behave, we froze the original transformer and captured separate low-rank adaptations (LoRA) of transformer weights:  One for adaptations originating from the mention-localization task and the other from the relation classification one.  We then plotted the adaptations of representative layers using a progressive color scale, showing their different trajectories.
    % In addition, we evaluated and visualized separating conflicting adaptations originating from different tasks by adopting low-rank adaptation (LoRA),  freezing the original transformer, and capturing adaptations originating from entity tasks vs. relation tasks into separate adapters. 
\end{description}

We perform ablation studies to attribute performance improvement to the various types of change and feature combinations. 

The remainder of this document is divided into sections, each corresponding to an area described above. Background, literature, and methods are addressed within each section to keep the content cohesive. 




==> 12A_AdditionalCapabilities.tex <==
In addition to the above capabilities, which have been implemented or are under development, the following list includes additional extensions under consideration.

\begin{description}
\item[Finetuning Strategy:] %DeBERTa-v3?
    Early finetuning runs through the pre-trained transformer with randomly initialized heads for the four tasks risks being destructive to lower layers of the model. A better fine-tuning strategy may entail a training protocol that initially freezes the transformer and then enables certain layer combinations to receive gradients as training progresses.
    \item[LoRA for MTL:] Low-Rank Adaptation (LoRA) is mostly considered a parameter-efficient fine-tuning method. It can also decouple incompatible task objectives back-propagating conflicting gradient updates in a multi-task setting. This can be achieved by freezing the shared encoder transformer and establishing different LoRA states for each competing task.
    \item[Meta-Learning:] Our current approach uses a simple meta-learner that calibrates thresholds for evaluation only. Can we find a way to efficiently use meta-learning techniques for training we may be able to generalize better and automate the tuning of additional hyperparameters? 
    \item[Data Imbalance:] Evaluate if weighting relation classification task losses (or their gradients) by class frequency improves performance and contributes to resolving the effects of class imbalance in the training dataset.
    \item[Coding Fixes:] We need to (1) complete some of the changes that are currently only applied to the joint model to also work with the single-objective models. (2) Rerun experiments and compile analysis. (3) Address discretionary items, such as compiling the model under PyTorch 2, which currently fails. (4) Cleanup code and publish the paper (at least part 1.)  
    
\end{description}

==> 20A_Literature.tex <==
\input{21D_ReDocRED.tex}
\input{21T_thresholding}
\input{21I_DataImbalance.tex}
\input{21M_MTL_TaskImbalanceI.tex}



==> 20B-Literature.tex <==
We cover three topics in this section, i.e., a description of the JEREX-L model, relevant work in Bayesian hyperparameter optimization, and relevant work in threshold calibration.
\input{23B-JEREX-L-Lit.tex}
\input{25B-HPO-Lit}
\input{28B-Threshold-Lit}



==> 21D_ReDocRED.tex <==

The DocRED dataset \cite{Yao2019DocREDAL} was designed for general document-level entity and relation extraction. According to the authors, it contains annotations for \num{132375} entities and \num{56354} relations that belong to 96 classes, \num{40.7}\% of which are inferred by synthesizing information from multiple sentences. This makes multi-sentence relation extraction much more challenging than similar single-sentence datasets like TacRED \cite{zhang2017tacred}. 

An effort to correct two problems with the DocRED led to the creation of the Re-DocRED \cite{tan2022revisiting} with \num{4053} documents re-annotated by humans raising the relation count to \num{120}K. 
The authors utilize two tests, i.e., \emph{Positive Relation Classification (PRC)} and \emph{Relation Extraction (RE)}, to analyze two types of errors that are found in DocRED:
\begin{description}
\item[False positives] are often observed with distant supervision generated annotations \cite{xiao-etal-2020-denoising} where database relations are matched on the entity pairs that appear in the passage, ignoring the context. Although such positive relations may generally be valid, they are sometimes unrelated to the text.%, leading to a high false positive rate.
\item[False negatives] are usually caused by missing or inconsistent annotations. Entities that should be related appear unrelated, and truly positive relations are evaluated as negative, based on the annotation \cite{tan2022revisiting}.  
\end{description}

They also compared relation extraction between DocRED and Re-DocRED, showing that state-of-the-art models, including JEREX, increase F1 scores by over 12 percentage points\footnote{The JEREX model used to arrive at these results appears to be the single-task relation extraction. Our Re-DocRED results are based on the Joint Multi-instance (MRC) Model and are generally lower than this value but still substantially better than the corresponding DocRED results}. 


It should be noted that similar revisions have been proposed for the popular single-sentence TacRED \cite{Stoica2021ReTACREDAS}.



==> 21I_DataImbalance.tex <==


\subsection{Background}

 Three issues often encountered in natural language classification tasks are: 
\begin{enumerate}
    \item \label{enum:easy-neg} In multi-label classification, when samples are heavily saturated with easy negative instances, while difficult ones are underrepresented, the model gets overwhelmed with trivial input and renders learning unproductive. 
        \cite{li-etal-2020-dice} 
        
    \item \label{enum:class-imbal}In multi-class classification, severe class imbalance skews a model's predictive bias so that it favors the majority classes.
    \item \label{enum:noisy} Data sources may contain erroneous or noisy examples, mislabeled or incorrectly formulated, that confuse and mislead the model's learning. In addition to fixing the annotations in the data, we are concerned with how to make the model more resilient, particularly when such errors are random and infrequent.   
\end{enumerate}

One class of approaches to address the undesirable effects of \autoref{enum:easy-neg} and \ref{enum:class-imbal} above is based on resampling the training input to become better-balanced \cite{Kulkarni2021FoundationsOD}. In an early influential study, Japkowicz \cite{Japkowicz2002TheCI} showed that the combination of \emph{the degree of imbalance} and \emph{the complexity of the concept}  determine the severity of the effect of data imbalance in classification. The skew is typically towards the negative samples, the majority class. At the same time, the complexity of the concept translates to difficulty in learning or uncertainty in prediction. These ideas lead to methods that address the problem algorithmically at the loss or gradient level.  

Algorithmic methods \cite{Fernndez2018LearningFI} have the flexibility to address complex situations, such as when balancing multiple outcomes in multi-label classification. \emph{Importance weighting} in deep learning \cite{Byrd2019WhatIT} adjusts losses to correct the imbalance in class distribution,  achieving similar results to resampling. However, this weighting is  more effective at the early stages of training since L2 regularization and batch normalization appear to reduce the need for importance weighting as training progresses \cite{Byrd2019WhatIT}. Many weighting techniques were proposed to improve object recognition in images (\autoref{enum:easy-neg} and \ref{enum:class-imbal}). Such techniques include \emph{Focal Loss} \cite{Lin2020FocalLF}, \emph{Asymmetric Loss} \cite{benbaruch2020asymmetric},  \emph{Distribution-Balanced Loss} \cite{Wu2020DistributionBalancedLF}. A method of weighting based on the \emph{Intersection-over-Union (IoU)} concept for natural language classification is \emph{Dice Loss} \cite{li-etal-2020-dice}. 

Other algorithmic methods operate at the gradient level to derive more precisely focused weights and directly manipulate gradients. Such proposals include \emph{Generalized Data Weighing} \cite{Chen2021GeneralizedDW},  \emph{Libra R-CNN} \cite{Pang2019LibraRT} for object detection in images. 


 

==> 21L-LearningRates.tex <==
\subsection{Background}

Partitioning model parameters into distinct groups with their own learning rates or other optimization hyperparameters is a common practice employed in both image and natural language models. As illustrated in \autoref{tab:paramGroups}, our parameter partitioning strategy focuses on learning rates (LR). The coarsest level (LR-0) divides the model into five distinct top-level groups, four of which correspond to specific tasks and one to the shared transformer component. Furthermore, we break down the shared transformer parameters into two subgroups (LR-1): one for the embedding module and another for the encoder. The encoder parameters can be further categorized based on the transformer layers (LR-2).

Additionally, we distinguish two L2 subgroups for each LR group, one containing those parameters subject to L2 regularization and the other those exempt from it. In keeping with the original JEREX implementation, embeddings, biases, and layer normalization parameters are excluded from L2 regularization corresponding to the sub-groups with ``No" in column L2.

\begin{table}
\centering
\begin{tabular}{lllr}
\textbf{LR-0} & \textbf{LR-1} & \textbf{LR-2} &  \textbf{L2} \\
\cmidrule(r){1-4}
\multirow[c]{4}{*}{Shared } & \multirow[t]{3}{*}{Embeddings}  & \multirow[c]{2}{*}{}  & No \\
& &  &  Yes \\
\cmidrule(r){2-4} 
 & \multirow[t]{3}{*}{Encoder}  & \multirow[t]{3}{*}{Layers 0-11}  & No \\
& &  & Yes \\

\cmidrule(r){1-4} 
\multirow[t]{3}{*}{Mention} &  &  & No \\
& &  &  Yes \\

\cmidrule(r){1-4}
\multirow[t]{3}{*}{Coreference} &  &  & No \\
& &  & Yes \\

\cmidrule(r){1-4}
\multirow[t]{3}{*}{Entity} &  &  & No \\
& &  & Yes \\

\cmidrule(r){1-4}
\multirow[t]{3}{*}{Relation} &  &  & No \\
& &  & Yes \\
\cmidrule(r){1-4}
\end{tabular}
\caption{Depiction of the parameter breakdown into three LR block levels, and whether they are subject to L2 regularization}
\label{tab:paramGroups}
\end{table}

For this research, we standardized the following parameter groupings:
\begin{description}
    \item[GLOBAL:] A global learning rate is used for all parameters, and a global weight decay value is used for all parameters subject to L2 regularization. Beyond these two values, we tune the weights used to combine the four task-specific losses into a multi-task loss, i.e., \emph{mention\_weight}, \emph{coref\_weight}, \emph{entity\_weight}, and \emph{relation\_weight}.
    \item[LR0-L2:] This partitioning has 10 parameters. Five independent learning rates are used for the \emph{LR0} groups and five weight decay rates for the respective parameter subgroups with \emph{L2=Yes}. To accommodate our TwinLoRA experiment discussed in section \ref{sec:twinLora}, a second learning rate is provided. So in technically, this grouping has 11 hyperparameters.    
    \item[LR1-L2:] This is the most granular partitioning with 18 parameters. Separate learning rates are used for L2-regularized and non-L2-regularized parameters in each of the \emph{LR1} groupings. Six independent weight decay values are used for the L2-regularized parameters. To accommodate our TwinLoRA experiment discussed in section \ref{sec:twinLora}, we allow a second set of four learning rates with different values. So technically, this grouping has 22 hyperparameters.
    \item[LR1-L2-TwinLoRA:]
\end{description}

By employing this meticulous partitioning strategy, we can fine-tune and optimize different segments of the model independently. 



==> 21M_MTL_TaskImbalanceI.tex <==
\subsection{Task Imbalance in MTL 
    \label{sec:MTL-opt}}

In multi-task learning (MTL), where some model components are shared among tasks, individual task losses may yield misaligned or conflicting gradients, exhibit high curvature, or be significantly different in magnitude  \cite{Yu2020GradientSF}. Since MTL training uses an aggregated loss, such conflicts may slow or prevent convergence. In addition, they often make it impossible to optimize all task objectives at once, changing the problem to one of selecting the component tasks that are more important to optimize. 

At the multi-task learning (MTL) level, where tasks share some parameter weights of upstream components, task losses are typically combined into an aggregate MTL loss used for optimization. Gradient descent over these shared weights uses linear combinations of individual task adjustments that often clash or point in opposite directions, and the optimization has difficulty converging. In their article ``Gradient Surgery for Multi-Task Learning"  \cite{Yu2020GradientSF}, the authors call a \emph{tragic triad} the confluence of three factors:: (1) conflicting gradients, (2) high curvature \footnote{Curvature is the inverse radius of the path  along the direction of the multi-task gradient between consecutive losses. High curvature is associated with steep transition}, and (3) a significant difference in gradient magnitudes. The authors propose \emph{PCGrad} that uses cosine similarity to detect and adjust conflicting gradients to address these three causes.  
\emph{Uncertainty-based regularization}  \cite{Kendall2018MultitaskLU,meshgi-etal-2022-uncertainty}, propose dynamically adapting task loss weighting based on the uncertainty reflected in the contributing task predictions. \emph{GradNorm} \cite{Chen2018GradNormGN},  directly normalizes and updates gradients based on the norm of a specifically chosen subset (usually the last layer) of shared parameters.
AutoLambda \cite{Liu2022AutoLambdaDD} is another adaptive method and a framework for multi-task learning that caries many significant weight-based implementations and gradient-based methods.
PC



==> 22A_ASL.tex <==
\subsubsection{Asymmetric Loss For Multi-Label Classification }
\label{sec:ASL}

%This section is based on \cite{Baruch2021AsymmetricLF}.

\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{media/ASL_plots_pos.png}
    \includegraphics[width=15cm]{media/ASL_plots_neg.png}
    \caption{We separate graphs with only positive (upper row) from those with only negative inputs (lower row). The two left plots show the computed ASL loss vs. logits ($z$) and vs. probabilities $p=\sigma(z)$, respectively.  Notice that in the negative case, the probabilities are shifted, suppressing the gradient's magnitude for true negative highly confident predictions, while $\gamma$ accentuates the relative effect of encouraging less confident false negative predictions.}
    \label{fig:galaxy1}
\end{figure*}

The binary cross-entropy loss for $K$ labels is:
\begin{equation}    
    L_\text{tot} = \sum_{k=1}^K L\left( \sigma(z_k),y_k \right) \label{eq:BCE} 
\end{equation}


Passing the logits $z_t$ produced by the classifier through the sigmoid function $\sigma(.)$ reduces them to probability-like values. The golden truth value $y_k$ can be  $1$ or $0$, denoting whether the real answer is true (positive) or false (negative). 

For each label $k$, we separate positive from negative losses:

\begin{equation}    
    L_k = -y_k L_k^+ - (1-y_k)L_k^-
\end{equation}

Assuming that the probabilities  $p_k = \sigma(z_k)$, these positive and negative cross entropy loss values are:

\begin{equation}  
\begin{cases}
    L_k^+ = \log(p_k) \\
    L_k^- = \log(1-p_k)
\end{cases}
\end{equation}

To convert these two losses to focal losses, we multiply them by a \emph{modulating factor} proposed by \cite{Lin2020FocalLF}

\begin{equation}  
\begin{cases}
    L_k^+ = (1-p_k)^\gamma \log(p_k) \\
    L_k^- = p_k^\gamma \log(1-p_k)
    \label{eq:focal}
\end{cases}
\end{equation}
The exponent $\gamma$ is a tunable focusing parameter. The focal loss modulating factor down-weighs extreme probabilities that correctly predict the outcome, i.e., high positive logits or low negative ones. The goal is to diminish high confidence losses that are correctly predicted while shifting the relative focus towards those less confident or those predicting the wrong outcome. Down-weighing the numerous easy examples that are correctly predicted prevents them from dominating learning. However, down-weighing positive examples that are correctly predicted  may weaken the model's  inductive bias towards those positive examples, which would be undesirable.

% \cite{Baruch2021AsymmetricLF}
To address this asymmetry \cite{benbaruch2020asymmetric} proposed a combination of \emph{asymmetric focusing} and \emph{asymmetric probability shifting}. Asymmetric focusing  entails splitting the focusing parameter into separate $\gamma^+$ and $\gamma^-$. Raising the $\gamma^-$ addresses the bias towards confidently predicted easy negative examples while leaving the $\gamma^+=0$ (or  a meager value)  allows the continuation of learning. 

Asymmetric probability shifting completely discards elementary negative examples whose probability is below a given threshold. The shifted probability $p'$ is calculated as follows:

\begin{equation}
    p'_k = \max(0, p_k-m)
\end{equation}

where $m \geq 0$ is the \emph{probability margin}

Probability shifting is equivalent to moving the probability curve to the right. It is an asymmetric variant of \emph{linear hinge loss} \cite{Bartlett2008ClassificationWA}, which introduces a third \emph{reject} outcome to a binary classifier that collects all results (logits) whose absolute value is less than a threshold $\delta$. 

Adding asymmetric focusing and probability shifting to equation \ref{eq:focal} we get the asymmetric loss ($L^\text{AS}$):

\begin{align}
L^\text{AS}_k &= -y_k L_k^+ - (1-y_k)L_k^- & 
\label{eq:asl-1}\\
\text{where} &:
\begin{cases}
    L_k^+ = (1-p_k)^{\gamma+} \,\log(p_k) \\
    L_k^- = (p'_k)^{\gamma-} \,\log(1-p'_k)
\end{cases}     \label{eq:asl-2}
\end{align}



==> 23A_DistributionBalancedLoss.tex <==
\subsubsection{Distribution-Balanced Loss }

\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{media/nt_bce_pos_plots.png}
    \includegraphics[width=15cm]{media/nt_bce_neg_plots.png}
    \caption{Positive example loss plots are shown for different values of class-specific bias $\nu$. Value $\nu=0$ is equivalent to  Cross-Entropy Loss (blue dash-dot lines). Since these are all examples with $y=1$, high model confidence towards a positive prediction needs no correction, while as confidence approaches zero, a proportionately greater magnitude negative correction is produced by the gradient 
Negative example loss plots are shown for different values of class-specific bias $\nu$ and scaling factor $\lambda$. Values $\nu=0$ and $\lambda=1$ are equivalent to the Cross-Entropy Loss (blue dash-dot lines). The dashed line shows what happens when we scale ($\lambda  \neq 1$) but not shift ($\nu=0$), while the dotted line shows the effect of shifting but no scaling. Since these are all examples with $y=0$, when the model shows very low confidence, the correction indicated by the gradient is negligible or zero. Otherwise, a correction is applied proportional to the model's confidence in predicting the wrong answer. How steep the increase depends largely on the scaling factor $\lambda$ while the bias $\nu$ shifts the curve to the right, suppressing the adjustment of easy negative examples that are confidently predicted correctly. }
    \label{fig:galaxy2}
\end{figure*}

The \emph{Distribution-Balanced Loss} (DBL) \cite{Wu2020DistributionBalancedLF}, is proposed as a replacement for \emph{Binary Cross-Entropy} (BCE) to address issues associated with label co-occurrence and negative label dominance in multi-label classification problems. Label co-occurrence manifests as cross-label correlations in the data that prevent simple weight-based down-sampling or up-sampling approaches from achieving a balanced representative distribution. That is unless they consider such co-occurrence patterns. 

For problems where $K$ instances, indexed by $k$ may belong to one, none, or many of a fixed number $C$  classes, indexed by $i$, a re-balancing weight factor $r_{i,k}$ is proposed to achieve optimal class balance:

\begin{align}
    P^C_i(x_k) &= \frac{1}{C} \frac{1}{n_i} &
    \label{eq:class-freq}\\
    P^I(x_k) &= \frac{1}{C} \sum_{y_{k,i} = 1} \frac{1}{n_i} & \label{eq:inst-freq}\\
    r_{k,i} &= \frac{P^C_i(x_k)}{P^I(x_k)}
    \label{eq:rebal-weight}
\end{align}

Equation \ref{eq:class-freq} determines the sampling frequency for a specific class $i$, as the product of the class probability times the probability of an instance belonging to that class. The value $n_i$ represent the number of instances that truly belong to class $i$.
Equation \ref{eq:inst-freq} returns the instance-level sampling frequency, i.e. how many truly positive samples are required for each instance on average. The ratio of these two quantities defines the re-balancing weight factor in equation \ref{eq:rebal-weight}. Based on this theoretical result, the authors propose equation \ref{eq:rebal-weight-hat} as a stable estimator for $r$\footnote{The authors chose $\alpha= 0.1$,
$\beta= 10$, and $\mu = 0.3$}:

\begin{equation}
    \hat{r}_{k,i} = \alpha + \frac{1}{1+exp\left(-\beta \times (r_{k,i} - \mu)\right)}
    \label{eq:rebal-weight-hat}
\end{equation}


The second aspect of the proposed \emph{distribution balanced loss} by \cite{Wu2020DistributionBalancedLF}  entails the \emph{negative-tolerant BCE} which is reshaped here to correspond to the structure of \ref{eq:asl-1}. %We distinguish classes, with count $C$, indexed by $i$, from instances that are indexed by $k$. For example, the DocRED dataset has $C=96$ classes of relations, and a given  example may have hundreds of candidate instances $K$ to classify. 

\begin{align*}
L_k^\text{NT-BCE} &= \frac{1}{C} \sum_{i=0}^C 
    \left[
    y_{k,i} L_{k,i}^+ + (1-y_{k,i}) L_{k,i}^-
    \right] & \nonumber\\
\text{where} &:
\begin{cases}
    L_{k,i}^+ = \log \left[1+e^{-(z_{k,i}-\nu_i)}\right] \\
    L_{k,i}^- = \frac{1}{\lambda}\log\left[1+e^{\lambda (z_{k,i}-\nu_i)}\right]
\end{cases}     %\label{eq:nt-bce0}
\end{align*}

Variables $\nu$ and $\lambda$ cause translation and scaling, aiming at a similar goal as $m$ and $\gamma$ of the asymmetric loss, only in the case of $L^\text{NT-BCE}$ they are operate on logits, before passing through the sigmoid function, while in the $L^\text{AS}$ case they operate on the generated probabilities. 
Using the sigmoid definition $p=\sigma(z)=\frac{1}{1+e^{-z}}$ we can express $L_k^\text{NT-BCE}$  in a way analogous to the asymmetric loss (equations \ref{eq:asl-1} and \ref{eq:asl-2}) at the class-instance level by eliminating the sum, reversing the log signs and rewriting the positive and negative losses as follows:
\begin{align}
L^\text{NT-BCE}_{k,i} &= -y_{k,i} L_{k,i}^+ - (1-y_k)L_{k,i}^- & \label{eq:nt-bce-1a} &\\
\text{where} &:
\begin{cases}
    p_{k,i} = \sigma(z_{k,i}-\nu_i) &\\
    p'_{k,i} = \sigma(\lambda (z_{k,i}-\nu_i)) &\\
    L_{k,i}^+ = \log(p_{k,i}) \\
    L_{k,i}^- =  \frac{1}{\lambda}\log(1-p'_{k,i})
\end{cases}     \label{eq:nt-bce-1b}
\end{align}

By replacing the logits with the corresponding probabilities we can easily see the similarities and differences between \ref{eq:nt-bce-1a} and \ref{eq:asl-1}.  
$\nu$, which controls the amount of shifting to the left (as $m$ does in the ASL) is dependent on the class. For cases such as DocRED relations where multiple instances are used per example and each instance is evaluated for membership in one of 96 classes, then the first two of equations \ref{eq:nt-bce-1b} indicate that there can be 96 different values of $\nu$, one for each relation type. Actually the authors propose an estimator for $\nu_i$ for each class $i$:

\begin{equation}
    \nu_i = \kappa \log(\frac{1}{p_i} - 1) 
\end{equation}

where $p_i = n_i/N$ is the probability that a random sample from $N$ instances will contain class $i$. The notation $n_i$ denotes the true count of instances that belong to class $i$. 

The $\nu$-shift is used in both the negative and positive examples, although the scaling parameter $\lambda$ is only applied on negative instances. 

By applying the balancing factor from equation \ref{eq:rebal-weight-hat} to $L^\text{NT-BCE}_{k,i}$ we get:

\begin{align}
L^\text{DB}_{k} &= \frac{1}{C} \sum_{i=0}^C \hat{r}_{k,i} \left[ -y_{k,i} L_{k,i}^+ - (1-y_k)L_{k,i}^- \right] & \label{eq:nt-bce-2a} &\\
\text{where} &:
\begin{cases}
    p_{k,i} = \sigma(z_{k,i}-\nu_i) &\\
    p'_{k,i} = \sigma(\lambda (z_{k,i}-\nu_i)) &\\
    L_{k,i}^+ = \log(p_{k,i}) \\
    L_{k,i}^- =  \frac{1}{\lambda}\log(1-p'_{k,i})
\end{cases}     \label{eq:nt-bce-2b}
\end{align}



==> 24A_Dice.tex <==
\subsubsection{Dice Loss for Data-imbalanced NLP Tasks}

Two issues associated with data imbalance that are handled neither by cross-entropy (CE) nor maximum likelihood estimation (MLE) are identified by \cite{li-etal-2020-dice}:
\begin{description}
    \item[Training-test discrepancy:] The learning process tends to bias learning towards the majority label. Each instance contributes equally towards the training objective at training time, thus favoring learning towards the most popular label. Testing, however, typically weighs positive and negative examples equally using the F1 score.  
    \item[Easy-negative example dominance:] A disproportionately large number of easy negative examples wastes the model's training cycles from learning to distinguish between positive and hard-negative examples. 
\end{description} 



==> 24A_FocalLoss.tex <==
\subsubsection{Focal Loss for Dense Object Detection \cite{Lin2020FocalLF}} 


==> 25A_MTL_GradNorm.tex <==
\subsubsection{GradNorm Adaptive Loss Balancing} \label{sec:gradnorm}



==> 26A_MTL_PCGrad.tex <==
\subsubsection{PCGrad  }\label{sec:PCGrad}

\emph{Projecting Conflicting Gradients (PCGrad)} \cite{Yu2020GradientSF} assumes $T$

==> 27A_MTL_UncertaintyWeightedLoss.tex <==
\subsubsection{Uncertainty-based-weighting}\label{sec:mtlUncertainty}
\label{sec:MTLuncert}
In addition to  task-specific losses $L_{\text{task}}^{(k)}$  we also compute uncertainty losses for each task $L_{\text{unc}}^{(k)}$. 
The computation of the multi-task loss is the weighted sum:
\begin{equation}
    %L = \frac{\sum_{k=0}^K w^{(k)} \left( L_{\text{task}}^{(k)} + \lambda %L_{\text{unc}}^{(k)} \right)} {\sum_{k=0}^K w^{(k)}}
    L = \sum_{k=0}^K w^{(k)} \left( L_{\text{task}}^{(k)} + \lambda L_{\text{unc}}^{(k)} \right)
    \label{eq:uncertLoss}
\end{equation}

Where $w^{(k)}$ are the fixed task weights used in the original JAREX implementation, $\lambda$ is a regularization parameter,  and $K$ is the number of tasks - four in our case. For each task $k$, the uncertainty loss calculation depends on the number of classes and labels involved. We base our approach on \cite{meshgi-etal-2022-uncertainty}
\begin{description}
    \item[Mention Localization]  is a binary multi-label classification with each candidate span treated as an independent label, with two possible classes: \emph{is a mention} and \emph{is not a mention}. A sigmoid function converts the logits produced by the classifier to confidence probabilities for each candidate. The uncertainty loss is then calculated as follows:
    $$
    L_{\text{unc}}^{(\text{men})} = \frac{1}{N^{\text{(men)}}}
    \sum_{i=1}^{N^{(\text{men})}} \zeta(x_i) 
    $$
    Where $N^{\text{(men)}}$ is the number of candidate mentions and $\zeta$ one of the uncertainty sampling functions discussed later in this section
    
    \item[Coreference Resolution] is also a binary multi-label classification of all possible pairs of recognized mentions. A sigmoid function converts the classifier output for each such pair to a probability expressing the confidence that its mentions are coreferent. The uncertainty loss is, again, calculated as follows:
    $$
    L_{\text{unc}}^{(\text{cor})} = \frac{1}{N^{\text{(cor)}}}
    \sum_{i=1}^{N^{(\text{cor})}} \zeta(x_i) 
    $$
    Where $N^{\text{(cor)}}$ is the number of mention-pairs, and $\zeta$ is one of the uncertainty sampling functions.
    
    
    \item[Entity Classification] is a multi-class classification where each candidate entity set representation is assigned a confidence probability for each entity type (class) using the softmax function. The uncertainty loss is calculated as follows:
    $$
    L_{\text{unc}}^{(\text{ent})} = \frac{1}{N^{\text{(ent)}}}
    \sum_{i=1}^{N^{(\text{ent})}} \zeta(x_i) 
    $$
    Where $N^{\text{(ent)}}$ is the number of entity representations and $\zeta$ one of the uncertainty sampling functions
    
    
    \item[Relation Classification] is treated as a multi-label multi-class classification. The classifier produces a binary confidence probability for each of the $N^{(\text{rel})}$  candidate relation representations (labels) for each of the $C$ relation types. The total number of instances evaluated are $C \times N^{(\text{rel})}$ for each example. The uncertainty loss is then calculated by averaging all instance uncertainties as follows:
    $$
    L_{\text{unc}}^{(\text{rel})} = \frac{1}{N^{\text{(rel)}}}
    \sum_{i=1}^{N^{(\text{rel})}} \left[ \overline{\zeta(x_i)}\right]_C
    $$
\end{description}

We next look into uncertainty sampling and the computation of the quantity $\zeta$ used in the above equations. For the intuition and theoretical underpinnings of uncertainty sampling, refer to \cite{KIUREGHIAN2009105}, \cite{Kendall2017WhatUD}
 and \cite{Kendall2018MultitaskLU}. We implemented three uncertainty sampling methods  following \cite{meshgi-etal-2022-uncertainty} with minor adjustments of the constant coefficients.   The simplest method is Least Confidence, \cite{settles-craven-2008-analysis}, which is defined as the complement of the highest probability over all classes in a multivariate distribution:
\[
\zeta_{\text{ LC}} = 1 - P_k(\hat{y}^{(1)}\mid x)
\]
We assume two classes (True and Not True) for binary multi-label classification for each label. 

The second method, i.e., Margin \cite{Scheffer2001ActiveHM}, depends on the difference between the two highest uncertainties among instances:

\[
\zeta_{\text{ M}} = 1 - P_k(\hat{y}^{(1)}\mid x) + P_k(\hat{y}^{(2)}\mid x)
\]

The third method is 
Shannon's entropy \cite{https://doi.org/10.1002/j.1538-7305.1948.tb01338.x}:

\[
\zeta_{\text{ H}} = -2 \sum_j \left[ P_k(\hat{y}^{(j)}\mid x) \log P_k(\hat{y}^{(j)}\mid x) \right]
\]



==> 30A_Data.tex <==
\subsection{Background}\label{sec:data}
\input{21D_ReDocRED}
\subsection{Dataset Comparison}
\input{51D_docred_redocred}
\subsection{Data in our Experiments}
\input{51E-ExperimentData}


==> 40A_Model.tex <==



==> 41B-OneEpochAllYouNeed.tex <==
In \cite{Egele2023IsOE}, Egele et al. propose a vertical approach to HPO, where many configurations are trained for one epoch, saving a checkpoint, and the best of them resume training. This sequential approach emulates what Hyperband does in parallel so that the most promising models complete the full cycle. 

==> 42A_Longformer.tex <==
% \subsection{Encoder Models}
\subsection{Bert Encoder Baseline}

We first established baselines for the joint task models and each single-task model using the initially proposed \emph{bert-base-cased} encoder by Eberts and Ulges \cite{eberts-ulges-2021-end}. 

\subsection{Longformer Encoder}

The alternative encoder model we chose for JEREX-L is the \emph{longformer-base-4096} transformer by \emph{The Allen Institute for AI} \cite{Beltagy2020Longformer}, which replaces the \emph{bert-base-cased} transformer \cite{DBLP:journals/corr/abs-1810-04805} of the original JEREX  implementation \cite{eberts-ulges-2021-end}. This change  
relaxes the 512-token size limitation BERT imposes on the input sequence. A length of 700 is safely above the most extended training example (623 tokens) in DocRED. However, the version of Longformer we chose allows up to 4K sequences, which is eight times longer than BERT's allowance.  

Instead of full self-attention, longformer implements a band-diagonal local attention matrix, also referred to as windowed attention, defined at initialization through the \emph{attention width} parameter. This approach decouples the length of the sequence from the maximum attention distance. It reduces the quadratic cost of self-attention (square of sequence length) to linear, proportional to the sequence length. Windowed self-attention works well when the valuable attending tokens are local and relatively close to their attended words. We assume that relations are more likely to have their head and tail entities within a sentence or two of a related mention.

In contrast, when resolving the coreferences of an entity, mentions can be further apart and may require attention to span several sentences. For this purpose, longformer employs \emph{global attention} in addition to local attention, whereby specified tokens can participate in bidirectional attention with all other global or local tokens. The tokens participating in global attention are passed as a parameter to the \emph{forward} method since they are likely to differ from  example to example. Combining local and global attention can maximize the benefits of self-attention over longer passages at a manageable cost. We introduced an option to set all tokens of nouns and proper nouns to participate in global attention and experimented with local attention window sizes ranging from 250 to 450 tokens.

\subsection{Other Encoders}

This research compares the original bert-base, and the longFormer alternative encoders described earlier. However, JAREX-L is adapted to take advantage of the auto-tokenizer and auto-model capabilities of Hugging Face, making it easy to try a variety of pre-trained transformers as encoders. We informally tried it, and it works with RoBERTa, Electra, and a few variants of Albert (albert-large-v2, albert-xlarge-v1, albert-xxlarge-v2).  



==> 51A_LinguisticAugmentation.tex <==
%\subsection{Linguistic Augmentation}

One of our hypotheses is that adding structural linguistic information to contextual embeddings generated by the encoder will enhance joint model performance. A similar approach is proposed in \cite{TYSS2021JointEA}. 

We added options to extract ``part-of-speech" (POS), ``dependencies" (DEP) and ``detailed English part-of-speech" tags (TAG) using the Spacy parser. The enabled types of codes are converted to fixed embedding vectors and appended to the hidden output of the encoder, before being used in any of the downstream representations of mentions, entities or relations. Enablement of the three optional linguistic augmentations as well as their embedding  size are controlled by optional model hyperparameters. 




==> 51C-ModelChanges.tex <==
\label{sec:RepChanges}

In the original JEREX model distance representation is implemented through embeddings reducing them to discrete categorical values with no notion of continuity. Specifically, edit distances in coreference resolution and token or sentence distances between pairs of entity mentions in relation classification were implemented this way. While the embedding approach can effectively interpret low-distance values, which are more frequent and thus amenable to generalization, it probably struggles with higher-distance values that occur less frequently, and the model is likely to succumb to mere memorization. 

Log-linear representations offer a superior alternative to embeddings for encoding distances.
The essence of these distances lies in the perception of affinity they signify between pair elements, which is non-linear and more faithfully conveyed by the logarithm of the distance. For instance, consider two pairs with distances of 1 and 2; the effective separation between these pairs is substantially more discernible than between pairs with distances of 344 and 345.

The superiority of log-linear representations in capturing and distinguishing these nuances in distance values lies both in the fact that they are continuous, and also in their ability to compress the range of values, emphasizing the significance of small differences and reducing the emphasis on large differences. In this way, they facilitate a more robust and interpretable representation of distances that is likely to enhance the performance of the coreference resolution and relationship classification task models.

A vector of pair distances $d$ of length $N$ can be represented as a matrix $D$ with shape $(N,1)$. We transform $D$ to a matrix $Z$ of shape $[N,E]$, like the original embedding solution, where $E$ is the embedding dimension size:
\begin{align*}
    Z = \log_2 (D+1) W^T
\end{align*}

$W$ is a weight matrix with dimensions $[E,1]$. This technique is used to represent coreference pair edit distances, relation pair token distances, and relation pair sentence distances. 

==> 51D_docred_redocred.tex <==
% Dataset Comparison

\begin{table}
\centering
\begin{tabular}{llr}
\toprule
 &  & \textbf{Doc} \\
\textbf{DocRED} & \textbf{ReDocRED} &  \textbf{Count} \\
\cmidrule(r){1-3}
\multirow[c]{2}{*}{test} & NA & 999 \\
 & val & 1 \\
 \cmidrule(r){1-3}
\multirow[c]{2}{*}{train} & train & 3052 \\
 & val & 1 \\
\cmidrule(r){1-3}
\multirow[c]{2}{*}{val} & test & 500 \\
 & val & 498 \\
 \bottomrule
\end{tabular}
\caption{ReDocRED contains the same examples as DocRED in its annotated training and validation splits. The table shows the \emph{almost} perfect alignment of training examples and how the DocRED-validation was split in half to form the ReDocRED dev and test. The DocRED-test is a blind dataset; its examples are not used in ReDocRED, except for one that ended up in the ReDocRED validation set.}
\label{tab:xtab2}
%\bottomrule
\end{table}
We compared three datasets: 
\begin{description}
    \item[DocRED:] This is the original dataset \cite{Yao2019DocREDAL}. It contains an annotated training split with  3053 examples, a validation with 998, a blind test set with 1000, and a  distant training one with 101873 examples that is outside our scope. 
    \item[DocREDJ:]  The DocRed-Joint, a slightly modified version by \cite{eberts-ulges-2021-end} used in the JEREX implementation. It consists of a training split with 3008 examples, a validation with 300, and a test with 700 examples.  
    \item[ReDocRED:] The revised new version \cite{tan2022revisiting} contains three splits: \emph{train} with 3053 examples, \emph{val}idation, and \emph{test} with 500 examples each. 
\end{description}
%The three datasets are based on the same document (example) pool but differ by how they are split. 
%We want to cross-calibrate our JAREX-L from ReDocRED, where it was trained, to DocRED.

\begin{table}
\centering
\begin{tabular}{lllr}
&  &  & \textbf{Doc} \\
\textbf{DocREDJ} & \textbf{DocRED} & \textbf{ReDocRED} &  \textbf{Count} \\
\cmidrule(r){1-4}
\multirow[c]{4}{*}{NA} & test & NA & 999 \\
\cmidrule(r){2-4} 
 & train & train & 29 \\
\cmidrule(r){2-4} 
 & \multirow[c]{2}{*}{val} & test & 9 \\
 &  & val & 6 \\
\cmidrule(r){1-4}
\multirow[c]{3}{*}{test} & train & train & 525 \\
\cmidrule(r){2-4} 
 & \multirow[c]{2}{*}{val} & test & 90 \\
 &  & val & 85 \\
\cmidrule(r){1-4}
\multirow[c]{5}{*}{train} & test & val & 1 \\
\cmidrule(r){2-4} 
 & \multirow[c]{2}{*}{train} & train & 2262 \\
 &  & val & 1 \\
\cmidrule(r){2-4} 
 & \multirow[c]{2}{*}{val} & test & 364 \\
 &  & val & 380 \\
\cmidrule(r){1-4}
\multirow[c]{3}{*}{val} & train & train & 236 \\
 \cmidrule(r){2-4} 
& \multirow[c]{2}{*}{val} & test & 37 \\
 &  & val & 27 \\
\end{tabular}
\caption{This three-way cross-tabulation shows how examples in the three splits of DocREDJ (the version used in the JEREX paper) map to their location in the official DocRED and ReDocRED.}
\label{tab:xtab3}
\end{table}

The cross-tabulation in \autoref{tab:xtab2} shows that both ReDocRED and DocRED share the same set of documents for training with one exception. The original set averaged $12.5$ triplets per document and underwent one re-annotation round to form the new ReDocRED training set, with $28.1$ triplets per document \cite{tan2022revisiting}. 

Notably, the Re-DocRED does not contain a blind test split. The $1K$ documents of the original DocRED validation set went through two rounds of re-annotations and were then split equally to form the ReDocRED validation and test sets. They average $34.6$ and $34.9$ triplets per document, respectively. This is a significant improvement compared to the $12.3$ annotated triplets average of the original validation set \cite{tan2022revisiting}.  

The extra round of re-annotations is a noteworthy difference between training and inference datasets. The authors attribute their tests' skew of precision-recall scores to this disparity. In our experiments, we considered compensating for this imbalance by optimizing the \emph{mention classifier threshold} to maximize a  micro-$F_{\beta} \, |\beta > 1$ score. However, after lengthy informal experimentation, we concluded that the  micro-$F_1$ performed best.\footnote{This study is not included in this document}


The three-way cross-tabulation in \autoref{tab:xtab3} shows how the document-to-split allocation for DocREDJ differs from  DocRED and ReDocRED.\footnote{For more detailed elaboration and analysis, see the \emph{nb\_Re\_DocRED\_differences} notebook provided with the code.}

%We created ReDocRED-compatible validation and test splits from the original DocRED validation examples according to their allocation in respective ReDocRED dataset splits. This way, we could evaluate and test on DocRED models trained on ReDocRED and vice-versa. This study does not include such cross-model evaluations. 



==> 51E-ExperimentData.tex <==
Our experiments use the dataset Re-DocRED \cite{tan2022revisiting}, which we have cached locally for convenience. The Huggingface dataset page is \href{https://huggingface.co/datasets/tonytan48/Re-DocRED}{tonytan48/Re-DocRED}. 

\autoref{tab:xtab2} shows two exceptions in mapping DocRED to Re-DocRED. Two DocRED documents, one from the test and the other from the training splits, ended in the ReDocRED validation split. We don't attempt to correct this discrepancy and prefer to use the datasets as defined. Since we never cross datasets between training and inference, this does not affect the validity of our results, and we never validate or test on data we used in training. 


==> 52A_LongformerEncoder.tex <==
\subsection{Longformer Encoder}

==> 53A_DataImbalance.tex <==
\subsection{Data Imbalance}
\input{22A\_ASL.tex}
\input{23A\_DistributionBalancedLoss.tex}
%\input{24A\_Dice.tex}

==> 54A_MTL-taskImbalance.tex <==
\subsection{Task Imbalance in MTL}\label{sec:MTL-imbalance}

The multi-task loss is calculated as the weighted sum of four component losses, (1) mention localization, (2) mention-pair coreference, (3) entity classification, and (4) relation classification. Instead of fixed weights, as in the original system, we consider two methods to improve multi-task-learning coordination. One is using  uncertainty-based weights \cite{Kendall2018MultitaskLU}.
The other is to use an adaptive loss balancing method such as GradNorm \cite{https://doi.org/10.48550/arxiv.1711.02257}, which normalizes component task gradients, or PCGrad, which adjusts conflicting grad vectors at every optimization step before summing them to form the multi-task gradient adjustment. 
%\cite{https://doi.org/10.48550/arxiv.2202.07281} % Multi-Task Interaction for ER Extraction using Selection Recurrent Network

For this analysis, we kept task loss calculations as defined in JEREX.

\begin{description}
    \item[Mention Localization]  is a binary multi-label classification with each candidate span treated as an independent label, with two possible classes: \emph{is a mention} and \emph{is not a mention}. A sigmoid function converts the logits produced by the classifier to confidence probabilities for each candidate. 
    \item[Coreference Resolution] is a binary multi-label classification of all possible pairs of recognized mentions. A sigmoid function converts the classifier output for each such pair to a probability expressing the confidence that its mentions are coreferent. Entities are defined in a multi-instance fashion, whereby the set of all coreferent mentions depicts the entity.
    \item[Entity Classification] is a multi-class classification where each entity belongs to exactly one entity type. The concatenation of mention and multi-instance representation forms the candidate entity representations. The softmax function assigns a confidence probability for each entity type (class) for each candidate entity (label). 
    \item[Relation Classification] is treated as a multi-label multi-class classification. The classifier produces a binary confidence probability for each of the $N^{(\text{rel})}$  candidate relation representations (labels) for each of the $C$ relation types. The total number of instances evaluated are $C \times N^{(\text{rel})}$ for each example. 
\end{description}



\input{27A_MTL_UncertaintyWeightedLoss.tex}
\input{25A_MTL_GradNorm.tex}
\input{26A_MTL_PCGrad.tex}





==> 54B_MTL-LoRA.tex <==
\subsection{Low-Rank Adaptation (LoRA)}\label{sec:twinLora}

Our implementation of LoRA in conjunction with freezing the transformer during training has two motivations:
of the conflicting gradient problem, we  

\begin{figure*}[htp]
    \centering
    \includegraphics[width=7cm]{media/lora_adaptation_differences-layer-0.png} \includegraphics[width=7cm]{media/lora_adaptation_differences-layer-11.png}
    \caption{LoRA weight adaptation captured under separate Entity and Relation adapters, showing the different adaptation trajectories caused by the gradients of the two tasks when decoupled}
    \label{fig:galaxy1}
\end{figure*}


==> 55A_MAML-Calibration-Outline.tex <==
\subsection{MAML with Calibration}\label{sec:autothreshLoop}

The regular test loop in \ref{alg:testLoop0} shows the baseline algorithm for training MAML model.  

\begin{algorithm}[hbt!]
\caption{MAML Inner-Outer Loops}\label{alg:testLoop}
\begin{algorithmic}
\Require{
    }    
\Ensure{}
\For{each Meta-Iteration}
    \State Sample Batch $B$ of tasks: $\{T^{(t)}\}$
    \For{$T=T^{(t)} \in B ; \forall(t) \in \abs{B}$ }
    \State $T = (S,Q) = (S^{(t)},Q^{(t)}) ; $ 
    \State Initialize $\phi \gets \theta$ ;
        \For{$(x_i,y_i) \in S$}
        \State loss $L_{i} = \mathcal{L}(\mathcal{M}(x_i \mid \phi),y_i)$
        \State $\phi \gets \phi - \alpha \nabla_{\phi} L_{i}$ ;
        \EndFor
    \EndFor
     \For{$q_i \sim p(\mathcal{D}^V)$}
        \State inner loop adaptation ;
    \EndFor
        \While{condition}   
  \If{condition}
   \State instructions1;
   \State instructions2;
  \Else
   \State instructions3;
  \EndIf
 \EndWhile
 \EndFor
\end{algorithmic}
\end{algorithm}

The regular test loop in \ref{alg:testLoop1} shows how prediction generation, thresholding, and scoring occur.  

\begin{algorithm}[hbt!]
\caption{Jerex-L MAML-Calibration Loop}\label{alg:testLoop}
\begin{algorithmic}
\Require{
        \begin{itemize}
        \item Datasets $\mathcal{D}^{tr}$, $\mathcal{D}^{val}$, $\mathcal{D}^{test}$ for sampling  $N^s$ support, $N^q$ query and $N^{mt}$ meta-test samples per meta-iteration $t$ respectively
        \item Initialize meta-parameters: $\theta$, $\eta$: meta-learning rate 
        \end{itemize}}    
\Ensure{support and meta-test pairs share classes}
\For{each Meta-Iteration}
    \State Sample batch of Tasks $\{T_i\}=(\{S_i\},\{Q_i\})$ 
    \For{each Task $T_i \in$ Batch}
    \State Initialize $\phi_i = \theta$ ;
%     \For{$(x_j,y_j) \sim p(\mathcal{D}^T)$}
        \For{$(x_j,y_j) \in S_i$}
        \State loss $L_{j,i} = \mathcal{L}(\mathcal{M}(x_j \mid \phi_{i}),y_j)$
        \State $\phi_i = \phi_{i} - \alpha \nabla_{\phi_i} L_{j,i}$ ;
        \EndFor
    \EndFor
     \For{$q_i \sim p(\mathcal{D}^V)$}
        \State inner loop adaptation ;
    \EndFor
        \While{condition}   
  \If{condition}
   \State instructions1;
   \State instructions2;
  \Else
   \State instructions3;
  \EndIf
 \EndWhile
 \EndFor
\end{algorithmic}
\end{algorithm}


==> 55B_CrossDatasetCalibration.tex <==
\subsection{Cross-Calibration Experiment}

\begin{table*}[htp]
 \centering
\begin{tabular}{lllrr}
\toprule
\textbf{Trained on} & \textbf{Calibrated} & \textbf{Tested on} & \multicolumn{2}{c}{\textbf{rel-nec-F1-micro}}  \\
 \textbf{Dataset} & \textbf{on Dev-Set} & \textbf{Test-Set} & \textbf{Dev}  & \textbf{Test}\\
 \cmidrule(r){1-5}
 \multirow[c]{1}{*}{Re-DocRED} & Re-DocRED & Re-DocRED &  50.14 & 47.57\\
      & DocRed & DocRED & 36.40  & 33.93\\
      & \color{gray}{DocRed-J} & \color{gray}{DocRED-J} & \color{gray}{53.73}  & \color{gray}{50.27} \\
      %& Re-DocRED-J-Dev & DocRED &   & \\
\cmidrule(r){1-5}
 DocRed-J & DocRed-J & DocRed-J & 44.49  & 38.90 \\
 \cmidrule(r){1-5}
 DocRed & DocRed & DocRed &   &  \\
\bottomrule
\end{tabular}
\caption{A model trained on Re-DocRED, calibrated thresholds on ReDocRED-dev, and testd on ReDocRED-test shows significantly better results than the same pipeline on DocRED-Joint or DocRED.  Cross-calibrating on DocRED the same model trained in Re-DocRED, as expected, is not performing as well as the models that were trained, calibrated and tested on data splits of the same distribution. The grayed row shows an illegitimate run where the ReDocRED model was cross-calibrated on DocRED-Joint-Dev, which overlaps with ReDocRED-Dev/Test) , the model trained, calibrated, and tested on DocRED-J.  \label{tab:cross-calib}}
\end{table*}

We trained a model on Re-DocRED-train for 25 epochs with auto-threshold on a rotating schedule. The rel-threshold was by category rather than a single value, i.e., a vector of 96 values. The rel-threshold started on epoch 11, the coref-threshold on epoch 15, and the mention on epoch 16. At the end of the training, we ran five consecutive threshold-tuning validations (threshold calibration) using the Re-DocRED-Dev dataset. We subsequently used the optimized thresholds on the Re-DocRED test set. The results are in the first line of \autoref{tab:cross-calib}. 

==> 70A_Analysis.tex <==
Discussion of what the results mean, what they don’t mean, where they can be improved, etc. These sections vary a lot depending on the nature of the paper. (For papers reporting on experiments with multiple datasets, it can be good to repeats Methods/Results/Analysis in separate (sub)sections for each dataset.)


==> 80A_Conclusion.tex <==
Quickly summarize what the paper did, and then chart out possible future directions that anyone might pursue.

==> 90A_ProjectLimitations.tex <==
For this section, imagine that your reader is a well-intentioned NLP practitioner who is seeking to make use of your data, models, or findings as part of a separate scholarly project, deployed system, or some other kind of real-world intervention. What should such a person know about your work? Especially important here are limitations and biases that might affect this person, their findings, their experiment participants, or the users of their product or service. The idea is that what you say here will be taken into consideration but this well-intentioned user, leading to better outcomes for everyone.



==> 95A_AuthorshipStatement.tex <==
Explain how the individual authors contributed to the project. Include whatever information you deem important to convey. For ideas and a model see \url{http://blog.pnas.org/iforc.pdf} (p.~12).

==> Notes-Multitask-Prefix.tex <==
User
Describe Prefix Finetuning, the parameter-efficient method of training a prefix for each task leaving the model frozen.

ChatGPT
Prefix finetuning is a parameter-efficient method used to train a prefix for specific tasks while keeping the rest of the model frozen. It is particularly useful when fine-tuning the entire model for each task would be computationally expensive or impractical. This approach allows for task-specific modifications to be made to the input and output layers of the model while keeping the intermediate layers fixed.

In prefix finetuning, the model is typically pre-trained on a large-scale dataset using a self-supervised or unsupervised learning objective. This pre-training phase helps the model learn general language representations and gain a broad understanding of various linguistic patterns and structures.

After the pre-training phase, the model is frozen, and a prefix is added to the model architecture. The prefix consists of task-specific input and output layers that are connected to the existing frozen layers of the model. The input layer of the prefix receives task-specific input features, such as task-specific tokens or metadata, which help the model understand the context of the task it needs to perform. The output layer of the prefix is designed to generate predictions or outputs specific to the given task.

The frozen layers of the model remain unchanged during prefix finetuning, which allows the model to leverage its pre-trained knowledge and linguistic understanding while adapting to the specific task requirements. By training only the prefix layers, the number of trainable parameters is significantly reduced compared to full model fine-tuning. This makes prefix finetuning more parameter-efficient and computationally less expensive.

During the finetuning process, the model is trained on task-specific labeled data, using a supervised learning objective that is appropriate for the task at hand. The gradients from the loss function computed for the prefix layers are backpropagated only through those layers, while the gradients do not flow through the frozen layers of the model.

By training only the prefix layers and keeping the rest of the model frozen, prefix finetuning strikes a balance between utilizing the pre-trained knowledge and adapting to specific tasks efficiently. It allows for rapid adaptation to new tasks without requiring extensive computational resources or retraining the entire model from scratch.





User
What is an example of how prefix layers are formed and integrated with the regular input to the frozen transformer

ChatGPT
Let's consider an example of using prefix layers to integrate task-specific information with the regular input in a frozen transformer model. Suppose we have a pre-trained transformer model that has been trained on a large corpus of text data.

For this example, let's assume our task is sentiment classification, where we want to determine whether a given text expresses positive or negative sentiment. We'll use the frozen transformer model and add a prefix layer specifically for sentiment classification.

Input Encoding:
The input to the transformer model is typically tokenized text. In the case of sentiment classification, we start by tokenizing the input text into a sequence of tokens. For example, the input sentence "I really enjoyed the movie" might be tokenized into ["I", "really", "enjoyed", "the", "movie"].

Prefix Layer:
We add a prefix layer to the model that is specifically designed for sentiment classification. This prefix layer will be connected to the regular input of the frozen transformer.

The prefix layer can include several components:

Task-specific Token: We add a task-specific token, such as "[SENTIMENT]", at the beginning of the token sequence. This token informs the model that the following text is related to sentiment classification.
Embedding Layer: The task-specific token, along with the regular tokens, goes through an embedding layer that maps each token to its corresponding dense vector representation. This layer is usually shared with the rest of the model.
Additional Features: Depending on the task, additional task-specific features can be incorporated. For sentiment classification, this could include features like the length of the input text or any other relevant metadata.
Integration with Frozen Transformer:
The output of the prefix layer is then concatenated with the regular input embeddings. The concatenated embeddings serve as the input to the frozen transformer layers.
During training, the frozen transformer layers remain fixed, and the gradients flow only through the prefix layers and the task-specific output layer. The prefix layers capture the task-specific information and adapt the input representation accordingly. The frozen transformer layers leverage their pre-trained knowledge and process the input to extract contextual representations.

Task-specific Output Layer:
After the frozen transformer layers, a task-specific output layer is added. In the case of sentiment classification, this output layer can be a dense layer followed by a softmax activation function, which produces a probability distribution over the sentiment classes (e.g., positive and negative).
During training, the parameters of the prefix layers and the task-specific output layer are updated, while the parameters of the frozen transformer layers remain fixed.

By adding and training the prefix layers while keeping the rest of the transformer model frozen, we can efficiently adapt the model to the specific sentiment classification task without retraining the entire model.





User
I want to use prefix tuning for four tasks in a multi-task model for entity-relation extraction. My current model uses a BERT transformer to receive paragraphs of text and outputs tensor h which is combined with additional features to form the input to the mention localization classifier, the co-reference resolution classifier that determines pairs of mentions that belong to the same entity, the entity classifier that determines the type of entities so formed and the relation classifier. I want to create a separate prefix for each task, and freeze the transformer. This way the four task objectives will appropriately adapt their own respective prefix and avoid gradient conflicts.

ChatGPT
Using prefix tuning for the four tasks in a multi-task model for entity-relation extraction is a great approach. Let's break down the steps to achieve this:

Base Model:
Your current model uses a BERT transformer to process paragraphs of text and produces tensor h, which serves as the base representation. This base model remains unchanged and frozen throughout the training process.

Task-specific Prefixes:
For each task (mention localization, co-reference resolution, entity classification, and relation classification), you will create separate task-specific prefixes. These prefixes will be integrated with the base representation h to adapt the model for each task.

Each task-specific prefix will consist of several components:

Task-specific Tokens: Start the input sequence with a task-specific token that identifies the task. For example, "[MENTION]" for the mention localization task, "[COREF]" for co-reference resolution, "[ENTITY]" for entity classification, and "[RELATION]" for relation classification.
Embedding Layer: The task-specific token, along with the regular tokens, passes through an embedding layer to obtain dense vector representations.
Additional Features: Include any additional task-specific features that are relevant to the respective task.
Integration with Base Model:
After the task-specific prefixes, the output embeddings are concatenated with the base representation tensor h from the BERT transformer. This concatenated input representation serves as the input for each task-specific classifier.

Task-specific Classifiers:
After the integration step, each task-specific classifier is added to the model architecture. These classifiers can be different dense layers or specific structures tailored to each task. For example, for mention localization, you can have a dense layer followed by a sigmoid activation function to predict the presence of a mention at each position in the input sequence. For co-reference resolution, you can use a binary classifier to predict whether pairs of mentions belong to the same entity.

Training:
During training, the base model (BERT transformer) remains frozen, and only the task-specific prefixes and classifiers are trained. This ensures that the gradients flow through the appropriate paths and avoid conflicts between tasks. Each task is trained with its respective objective using labeled data specific to that task.

By using separate prefixes and freezing the base model, you enable each task to adapt independently without interfering with the others. This approach allows for efficient multi-task learning for entity-relation extraction while leveraging the pre-trained knowledge from the BERT transformer.





User
Let's say the input to the current model is a token sequence, without special tokens, that is fed to the BERT encoder. Now we introduce a new special token that can represent [MENTION], [COREF] etc.. These special tokens have to be introduced to the tokenizer since they will be processed through the transformer, right?

ChatGPT
Yes, that's correct. When introducing new special tokens such as [MENTION], [COREF], and so on, they need to be added to the tokenizer so that they can be properly processed by the transformer model.

The tokenizer plays a crucial role in tokenizing the input text into a sequence of tokens and converting those tokens into numerical representations that can be fed into the transformer encoder. It handles the mapping between the textual input and the tokenized input understood by the model.

To incorporate the new special tokens, you would need to modify the tokenizer to recognize and tokenize them accordingly. Here's a general overview of the steps:

Add Special Tokens: Extend the tokenizer's vocabulary to include the new special tokens, such as [MENTION], [COREF], [ENTITY], [RELATION], or any other tokens specific to your tasks. These tokens should be unique and distinct from the existing tokens in the vocabulary.

Tokenization: When tokenizing the input text, the tokenizer will recognize the special tokens based on their textual representation. For example, if the input sequence contains "[MENTION]", the tokenizer should identify it as a single token rather than treating each character individually.

Token IDs: Assign unique token IDs to the special tokens in the tokenizer's vocabulary. These token IDs will be used to represent the special tokens numerically in the input sequence.

Input Encoding: Encode the token sequence into numerical representations that can be fed into the transformer encoder. The tokenizer will convert each token, including the special tokens, into its corresponding token ID.

By incorporating the special tokens into the tokenizer and adjusting the vocabulary and encoding process, you ensure that the special tokens are properly processed by the transformer model during inference and training. This allows the model to recognize and utilize the task-specific information encoded by the special tokens in the prefix layers and downstream task-specific classifiers.





User
But the pre-training did not include such special tokens, so they will be unknown to the model. Also, the token-ids should not replace existing token-ids so that the token-to-token-id mapping is the same as when the transformer was trained

ChatGPT
You're correct, and I apologize for the confusion in my previous response. If the pre-training of the transformer model did not include the special tokens, they will be unknown to the model, and simply adding them to the tokenizer's vocabulary and using new token IDs would not be sufficient.

To ensure compatibility with the pre-trained transformer model, you should consider an alternative approach:

Special Tokens as Regular Words: Instead of introducing new special tokens, you can treat the task-specific markers (e.g., [MENTION], [COREF], etc.) as regular words within the token sequence. This means they will be tokenized and encoded just like any other word in the input text.

Encoding Task Information: Rather than relying on special tokens, you can encode the task-specific information as part of the input sequence itself. For example, you could prepend each input sentence with a task-specific marker, such as "MENTION: I really enjoyed the movie" or "COREF: The two actors performed exceptionally well." This way, the task-specific information is embedded directly within the text, and the pre-trained transformer model can process it as regular input.

Adaptation via Prefix Layers: Instead of adding new special tokens, you can use prefix layers to incorporate the task-specific information. The prefix layers, which we discussed earlier, can process the input sequence and adapt it based on the task requirements without modifying the original tokenization or introducing unknown tokens to the pre-trained model.

By encoding task information directly within the input text and using prefix layers for adaptation, you can ensure compatibility with the pre-trained transformer model. This way, the token-to-token ID mapping remains consistent with the pre-training and the model can leverage its pre-trained knowledge while adapting to the specific task at hand.





User
This sounds like a hard prefix solution, not a soft one.

ChatGPT
Apologies for the confusion. You're right, the approach I described earlier aligns more closely with a hard prefix solution rather than a soft one. In a hard prefix approach, the task-specific information is explicitly encoded within the input sequence.

For a soft prefix solution, which allows for more flexibility and compatibility with the pre-trained model, you can use the following approach:

Special Tokens and Tokenization: Introduce the special tokens (e.g., [MENTION], [COREF], etc.) to the tokenizer's vocabulary. These tokens should be distinct and unique.

Input Encoding:

When encoding the input sequence, add the relevant special tokens at appropriate positions to indicate the task-specific context. For example, you can prepend the input sequence with the [MENTION] token to indicate the mention localization task.
During tokenization, the special tokens will be split into sub-tokens based on the tokenizer's rules. For example, [MENTION] might be tokenized into "[", "MENT", "##ION", "]" using BERT's WordPiece tokenization.
The resulting sub-tokens, including the special tokens, will have corresponding token IDs based on the tokenizer's vocabulary.
Prefix Layers:

In the model architecture, create separate prefix layers for each task. These prefix layers should handle the special tokens and process them accordingly.
The prefix layers can include task-specific embeddings, additional features, or any other modifications required for each task.
Integration with Frozen Transformer:

Concatenate the output of the prefix layers with the token embeddings produced by the frozen transformer layers.
This concatenated representation will serve as the input to the task-specific classifiers.
Training:

During training, only the prefix layers and the task-specific classifiers are updated, while the frozen transformer layers remain fixed.
Each task is trained with its respective objective using labeled data specific to that task.
By employing a soft prefix solution, the special tokens are recognized and tokenized by the tokenizer, ensuring compatibility with the pre-trained model. The prefix layers then handle the task-specific information and adapt the input accordingly while integrating with the frozen transformer layers. This approach allows for more flexibility in incorporating task-specific context without introducing incompatible tokens or modifying the pre-trained model's token-to-token ID mapping.





User
can you give me an example of these prefix layers, say for MENTION and COREF

ChatGPT
Certainly! Here's an example of how the prefix layers can be structured for the MENTION and COREF tasks in a soft prefix solution:

MENTION Prefix Layer:

Task-specific Token: The input sequence for the MENTION task can be prepended with the special token [MENTION].
Token Embedding: The [MENTION] token, along with the rest of the tokens in the input sequence, passes through an embedding layer that maps each token to its dense vector representation.
Additional Features: Depending on the requirements of the MENTION task, you can incorporate additional features such as the length of the input text or any other relevant metadata.
COREF Prefix Layer:

Task-specific Token: For the COREF task, prepend the input sequence with the special token [COREF].
Token Embedding: The [COREF] token and other tokens in the input sequence are processed by the embedding layer to obtain their dense vector representations.
Additional Features: Include any additional features specific to the COREF task that might aid in co-reference resolution, such as the position of the tokens in the input sequence.
Both MENTION and COREF prefix layers follow a similar structure with task-specific tokens, token embeddings, and additional features. These prefix layers allow the model to adapt the input representation for each task while leveraging the pre-trained transformer's knowledge encoded in the frozen layers.

The output of the prefix layers can be concatenated with the token embeddings produced by the frozen transformer layers. This concatenated representation serves as the input to the respective task-specific classifiers, which can be dense layers or task-specific structures tailored to the MENTION and COREF tasks.

During training, the prefix layers and task-specific classifiers are updated while the frozen transformer layers remain fixed, ensuring that the model adapts to the specific objectives of each task without modifying the pre-trained transformer's token-to-token ID mapping or introducing incompatible tokens.





User
What type of module are the prefix layers? Does their output become input to the transformer?

ChatGPT
The prefix layers can be implemented as a combination of various modules, depending on the specific requirements of your model architecture. Here are a few commonly used modules that can be part of the prefix layers:

Embedding Layer: The embedding layer maps each token (including the special tokens) to its corresponding dense vector representation. This layer is typically shared with the rest of the model, including the transformer layers.

Additional Feature Layers: If you have additional features specific to the task, such as the length of the input text or position information, you can incorporate separate layers to process and integrate these features into the prefix layers. These layers can be fully connected layers, convolutional layers, or any other appropriate modules based on the nature of the features.

Attention Layers: Depending on the requirements of the task, you may include attention layers within the prefix layers. These attention layers can capture task-specific contextual dependencies and relationships between the tokens in the input sequence.

The output of the prefix layers, after processing through the various modules, can be concatenated with the token embeddings produced by the frozen transformer layers. This concatenated representation serves as the input to the transformer layers.

The frozen transformer layers then process this input to extract contextual representations, incorporating both the pre-trained knowledge from the transformer and the task-specific information introduced by the prefix layers. The output of the transformer layers can subsequently be passed to task-specific classifiers or other downstream layers for further processing or prediction.

In summary, the prefix layers consist of various modules such as embedding layers, additional feature layers, and possibly attention layers. Their output, along with the token embeddings, becomes the input to the frozen transformer layers, allowing for the integration of task-specific information with the existing transformer model.





User
So the prefix layer constitutes a block with an output that includes the sequence length and embeddings as dimension?

ChatGPT
Yes, the prefix layer can be viewed as a block that takes the input sequence, including the special tokens, and processes it to produce an output representation. The output of the prefix layer would typically include the following dimensions:

Sequence Length: The length of the input sequence is an important dimension in the output of the prefix layer. It represents the number of tokens in the sequence, including both the special tokens and the regular tokens.

Embeddings: The prefix layer applies an embedding layer to map each token in the input sequence to its corresponding dense vector representation. The output of the embedding layer would include the embeddings for all tokens, including both the special tokens and the regular tokens. The embedding dimension would depend on the chosen embedding size or the pre-trained embedding model used.

Additionally, depending on the specific requirements of the task and the design of the prefix layer, the output may also include other dimensions or additional features relevant to the task. For example, if the task requires positional information, the output might include the position embeddings for each token.

In summary, the output of the prefix layer consists of the sequence length and the embeddings for each token in the input sequence, including the special tokens. These dimensions capture the task-specific information and serve as input to the subsequent frozen transformer layers for further processing.





User
And this prefix block output is input to the transformer?

ChatGPT
Yes, that's correct. The output of the prefix layer, which includes the sequence length and embeddings for each token in the input sequence (including the special tokens), is used as input to the subsequent frozen transformer layers.

The prefix block output, along with the token embeddings produced by the prefix layer, is concatenated and forms the input to the transformer layers. This concatenated representation incorporates both the task-specific information introduced by the prefix layers and the pre-trained knowledge encoded in the transformer.

The frozen transformer layers process this input, capturing contextual information and relationships between tokens to produce contextualized representations. These representations contain a combination of the pre-trained knowledge from the transformer and the task-specific adaptations from the prefix layers.

The output of the transformer layers can then be passed to task-specific classifiers or other downstream layers for further processing or prediction related to the specific tasks in your multi-task model.





User
I am not sure about whether we should create special tokens or let the model break-up the special tokens based on its pre-training. The transformer is pre-trained without these special tokens.

ChatGPT
Apologies for the confusion. You are correct in considering the pre-training setup of the transformer model. If the transformer model was pre-trained without the special tokens, it's advisable not to introduce new special tokens that the model is unfamiliar with.

Instead, you can encode the task-specific information implicitly within the input sequence without relying on special tokens. This can be achieved by modifying the input text or using an alternative approach. Here's an example:

Implicit Encoding:
For the MENTION task, you can modify the input text by incorporating task-specific markers within the sentences. For instance, you could prepend each sentence that contains a mention with a marker like "MENTION: ". This allows the model to implicitly identify the mention-related context without introducing unknown tokens.
Similarly, for the COREF task, you can prepend sentences that indicate a coreference relationship with a marker like "COREF: ".
By modifying the input text in this manner, the task-specific context is embedded implicitly within the sentences, and the pre-trained transformer can process them as regular input. The transformer can leverage its existing knowledge to capture task-specific information without encountering unfamiliar tokens.

You can then proceed to integrate the modified input text with the transformer model, with the prefix layers adapting and processing the input accordingly. The output of the prefix layers, along with the token embeddings produced by the frozen transformer layers, would serve as input to the downstream task-specific classifiers.

Remember to align the training process such that the prefix layers and task-specific classifiers are updated while keeping the frozen transformer layers fixed, ensuring that the model adapts to the specific task objectives while leveraging the pre-trained knowledge of the transformer model.





User
So we have four tasks. We should create four copies of the input sequence and prefix each one with a keyword (like MENTION, COREF, ENTITY, RELATION). The four versions of the input will then be processed through the prefix block, assigning embeddings, going through two linear layers (an activation?) and feeding the result to the transformer. 

ChatGPT
Yes, your understanding is correct. In the case of having four tasks (MENTION, COREF, ENTITY, RELATION), one approach is to create four copies of the input sequence, each prefixed with a corresponding keyword to indicate the task context.

Here's a step-by-step breakdown of the process:

Input Preparation:

Take the original input sequence.
Create four copies of the input sequence, one for each task (MENTION, COREF, ENTITY, RELATION).
Prepend each copied sequence with a task-specific keyword, such as "MENTION:", "COREF:", "ENTITY:", "RELATION:", respectively. This keyword acts as an implicit marker for the task context.
Prefix Block Processing:

Process each modified input sequence, including the task-specific keyword, through the prefix block.
The prefix block includes layers such as an embedding layer, linear layers (potentially with activation functions), and any other relevant modules specific to each task.
The prefix block assigns embeddings to the tokens, applies transformations, and captures task-specific information.
Transformer Integration:

Concatenate the output of the prefix block, which includes the token embeddings and processed task-specific information, with the token embeddings produced by the frozen transformer layers.
This concatenated representation, which combines the task-specific context from the prefix block with the pre-trained transformer knowledge, becomes the input to the subsequent layers of the model.
Further Processing and Prediction:

Pass the concatenated representation through the frozen transformer layers to capture contextualized representations and leverage the pre-trained knowledge.
The output of the transformer layers can be passed to task-specific classifiers or other downstream layers for further processing or prediction related to each task.
By creating task-specific copies of the input sequence and prefixing them with keywords, you establish the task context implicitly. The prefix block processes each modified input sequence to capture task-specific information before integrating with the frozen transformer layers.

This approach allows the model to adapt to the specific requirements of each task while benefiting from the pre-trained transformer's knowledge.





User
It seems that adding the keywords MENTION, COREF, ENTITY and RELATION is not necessary, since the losses will backpropagate to their copy of the prefix block

ChatGPT
You are correct. I apologize for the confusion caused by the unnecessary inclusion of keywords in each input sequence. In a multi-task setting, where you have separate copies of the prefix block for each task, there is no need to include explicit keywords like "MENTION," "COREF," "ENTITY," or "RELATION" in the input sequences.

The separate copies of the prefix block associated with each task already provide the task-specific context implicitly. The losses for each task will backpropagate through their respective prefix block, allowing each task to adapt its own set of parameters without the need for explicit keywords.

Therefore, you can skip the step of adding keywords to the input sequences. Simply create separate copies of the input sequence for each task, pass them through their respective prefix blocks, and integrate the outputs with the frozen transformer layers as previously described. This approach allows each task to adapt independently while leveraging the pre-trained transformer's knowledge.





User
At the end of each prefix block, should we add a ReLU or other type of activation?

ChatGPT
The choice of whether to include an activation function, such as ReLU or any other type, at the end of each prefix block depends on the specific requirements and characteristics of your model and tasks. Here are a few considerations:

Task-specific Requirements: Consider the nature of the task and the desired behavior of the prefix block's output. If the task requires non-linearity or certain activation patterns, you may choose to include an activation function to introduce non-linear transformations. For example, tasks like sentiment analysis or named entity recognition may benefit from activation functions like ReLU to capture non-linear relationships in the data.

Model Complexity: Adding activation functions increases the model's capacity to learn complex patterns, but it also introduces additional non-linearities that can make training more challenging. Consider the complexity of your tasks and the available training data when deciding whether to include an activation function.

Gradient Flow and Stability: Activation functions can affect the gradient flow during backpropagation. Some activation functions, such as ReLU, can help alleviate the vanishing gradient problem by allowing gradients to flow more easily. However, they can also lead to the dying ReLU problem, where a large portion of activations becomes zero. It's important to monitor the gradient flow and the behavior of the model during training to ensure stability and prevent issues like gradient saturation or instability.

In many cases, the choice of whether to include an activation function at the end of the prefix block will depend on empirical experimentation and the specific characteristics of your tasks and data. It's recommended to try different configurations, including with and without activation functions, and evaluate their impact on performance and convergence during training.

Additionally, you can consider other architectural choices, such as using normalization layers (e.g., batch normalization) or skip connections, to further enhance the model's performance and stability.





User
I am afraid that adding an activation function at the end of the prefix block and before passing the result to the transformer as input, may interfere with the pre-training of the frozen transformer and obfuscate the meaning of these embeddings

ChatGPT
You are correct in your concern that adding an activation function at the end of the prefix block, before passing the result to the frozen transformer, could potentially interfere with the pre-training of the transformer and affect the interpretation of the embeddings.

When using a pre-trained transformer model, the embeddings produced by the transformer have specific meanings and capture contextual information that has been learned during pre-training. Introducing an activation function immediately before passing the output to the transformer can alter the distribution and interpretation of these embeddings, which may not align with the pre-training objectives.

To preserve the integrity of the pre-trained embeddings and ensure compatibility with the pre-training setup, it is generally recommended to avoid inserting activation functions directly before the frozen transformer layers.

Instead, you can consider incorporating the activation functions or non-linearities within the prefix block itself, before producing the final output. By doing so, you allow the task-specific adaptations within the prefix block to capture non-linear relationships and process the input sequence while keeping the transformer embeddings intact.

Once the output of the prefix block is obtained, it can be concatenated with the pre-trained embeddings from the frozen transformer layers without further activation functions. This ensures that the pre-trained embeddings retain their original meaning and are compatible with the frozen transformer.

Remember, the goal is to adapt the model to specific task objectives without compromising the pre-trained knowledge encoded in the transformer. By carefully designing the prefix block and avoiding interference with the pre-trained embeddings, you can strike a balance between task-specific adaptation and leveraging the transformer's pre-training.





User
Could I use a BERT layer block as the prefix block? This way it will be like allowing each task to have their own first block in a 13-layer transformer, with the 12 layers following the first being frozen and pretrained

ChatGPT
Yes, you can use a BERT layer block as the prefix block for each task in your multi-task model. This approach allows each task to have its own initial block in a 13-layer transformer, with the subsequent 12 layers being frozen and pretrained.

Using a BERT layer block as the prefix block provides several benefits:

Consistency with Pretraining: Since BERT is a widely used and well-established transformer model, using a BERT layer block ensures consistency with the pretraining setup. The pretrained BERT layers capture general language understanding, and by including a BERT layer as the prefix block, you align the architecture with the same transformer model used during pretraining.

Task-specific Adaptation: The prefix block, consisting of the BERT layer block, can be fine-tuned and adapted to the specific task at hand. By allowing each task to have its own initial block, you enable task-specific adaptation within the prefix layers while leveraging the pretrained knowledge encoded in the remaining frozen transformer layers.

Parameter Efficiency: Freezing the subsequent 12 layers of the transformer and only adapting the prefix block provides parameter efficiency. It reduces the number of trainable parameters and enables sharing of pre-trained knowledge across tasks while still allowing task-specific adaptation in the prefix layers.

Remember to align the training process so that the prefix block and task-specific layers are updated during fine-tuning while keeping the remaining transformer layers frozen.

By using a BERT layer block as the prefix block, you maintain consistency with pretraining, allow task-specific adaptation, and leverage the parameter efficiency of a pretrained transformer model.





User
I was thinking I would use BERT for the version of the model that uses BERT as the transformer. I have another version that uses LongFormer for longer inputs and taking advantage of the local/global attention. For the LongFormer model I was thinking of using a Roberta or single-layer longformer for the prefix block

ChatGPT
Using a BERT layer block as the prefix block for the version of the model that uses BERT as the transformer is a reasonable choice. BERT's architecture aligns well with the pretrained BERT transformer, ensuring consistency and leveraging the pretraining setup.

For the version of the model that uses LongFormer as the transformer to handle longer inputs and utilize local/global attention, you can consider using a single-layer Longformer or a Roberta model as the prefix block. Both choices can work effectively in this scenario.

Single-layer Longformer: Utilizing a single-layer Longformer as the prefix block aligns with the Longformer transformer architecture used in the main model. It allows the prefix block to adapt to the task-specific requirements while maintaining consistency with the main model's design.

Roberta: Alternatively, using a Roberta model as the prefix block can be beneficial. Roberta is a variant of BERT that applies modifications to improve performance and efficiency. It can serve as an effective prefix block, providing task-specific adaptation while leveraging the pretraining of the Roberta model.

Both options allow you to incorporate the benefits of the Longformer model and its attention mechanisms while adapting the prefix block specifically to your tasks.

Remember to keep the remaining layers of the LongFormer transformer frozen during training to retain the benefits of the pretraining process and ensure the main model's architecture remains intact.

By using a single-layer Longformer or a Roberta model as the prefix block in the LongFormer version of your model, you can achieve task-specific adaptation while leveraging the benefits of the Longformer transformer for longer inputs and local/global attention.





User
Let's say I setup four prefix blocks named prefix_mention, prefix_coref, prefix_entity, and prefix_relation. I will use one frozen transformer shared for all tasks. I will need to distinguish the four outputs of this transformer that corresponds to each of the prefix_blocks feeding it. So I will probably have to define four sequence modules, with each of the prefix blocks and the same encoder transformer.  I will then have to process each of these separately to produce each of the h outputs that feed the respective tasks. Is there a better way to share the transformer and process all inputs with one pass?

ChatGPT
Yes, you can share the frozen transformer across all tasks and process all inputs with one pass to improve efficiency. Rather than defining separate sequence modules for each prefix block, you can use a single sequence module that accepts all input sequences for all tasks simultaneously. This allows you to process all inputs in parallel and obtain the respective outputs for each task in one pass through the transformer.

Here's a suggested approach to achieve this:

Combine Input Sequences:

Concatenate all the input sequences from different tasks into a single batch, ensuring the sequences are appropriately padded to the maximum length within the batch.
The combined input sequences would include the input for all four tasks (MENTION, COREF, ENTITY, RELATION) in a single tensor.
Process Inputs with Shared Transformer:

Pass the combined input sequences through the shared frozen transformer. This can be done in one forward pass.
The output of the transformer will contain representations for all input sequences, including those from all four tasks.
Extract Task-Specific Outputs:

After processing the combined input sequences with the transformer, you can extract the task-specific outputs by indexing or slicing the transformer output based on the corresponding positions of each task's input sequences.
This way, you can obtain the specific representations (h outputs) for each task from the shared transformer output.
By processing all inputs together in a single pass through the shared transformer, you can take advantage of parallel computation and improve efficiency. Extracting the task-specific outputs from the shared transformer output allows you to obtain the representations needed for each task without requiring multiple passes through the transformer.

Remember to adjust the subsequent layers or classifiers after extracting the task-specific outputs to align with the specific requirements of each task.

This approach enables the sharing of the transformer and allows for simultaneous processing of inputs, reducing computational overhead and improving efficiency in your multi-task model.





User
I am not sure I understand what you propose. All inputs to the four prefix blocks is identical: the input text passage. Each of the prefix blocks may produce a slight variation of encodings that should be fed to the transformer. I see two ways to combine the four inputs. One is to concatenate the sequences and pass a sequence of four times the size of the input text, which will severely limit the allowed size of my input which is already tight. Another approach is to add a "task" dimension to the batch, which will now have shape [batch, task,seq, embedding] where the task dimension is always 4. I can unravel these four entries and send each h output  to the respective task classifiers.

ChatGPT
Apologies for the confusion. I misunderstood your setup initially. Based on your clarification, it seems that the inputs to the four prefix blocks are indeed identical, and each prefix block may produce a slightly different encoding that needs to be fed into the shared transformer.

In this case, your approach of adding a "task" dimension to the batch is appropriate. By adding a task dimension, you can process the inputs in parallel while preserving their individuality. Each prefix block's output can then be unraveled and fed to their respective task classifiers.

Here's a revised overview of the approach:

Inputs:

The input text passage is the same for all four tasks.
Prefix Blocks:

Create four separate prefix blocks: prefix_mention, prefix_coref, prefix_entity, and prefix_relation.
Each prefix block processes the input text passage and produces a task-specific encoding.
Combine Inputs:

Add a "task" dimension to the batch, resulting in a tensor of shape [batch, task, seq, embedding].
Each task-specific input will have its own dimension along the task axis, allowing differentiation between the tasks.
Shared Transformer:

Pass the combined inputs through the shared frozen transformer, considering the "task" dimension.
The shared transformer processes all task-specific inputs simultaneously, leveraging parallel computation.
Extract Task-Specific Outputs:

Unravel the shared transformer output along the "task" dimension to obtain the individual task representations.
Each task-specific output can be fed into its respective task classifier for further processing.
By adding the "task" dimension to the batch and processing the inputs in parallel, you can leverage the shared transformer for efficient computation. Extracting the task-specific outputs from the shared transformer output allows you to feed each task's representations to their respective classifiers.

This approach enables you to share the transformer across tasks, process the inputs in parallel, and maintain the individuality of each task's encoding without the need for concatenating the sequences or limiting the input size.

I apologize for any confusion caused earlier, and I hope this revised explanation clarifies the approach for your multi-task model.





User
So now I have to find an efficient way to load and initialize the four prefix blocks as single-layer transformers. Should I initialize them to the equivalent of an identity or random? It seems that at first it would make sense to keep the input intact as the transformer would see it if no prefix block were involved.

2 / 2


ChatGPT
When initializing the four prefix blocks, a reasonable approach would be to initialize them to an equivalent of an identity or keep them as close as possible to the original input representation. This initialization helps ensure that the prefix blocks initially do not introduce significant changes to the input and allow the transformer to process it as if no prefix blocks were involved.

There are a few possible ways to achieve this:

Identity Initialization: Initialize the weights of the prefix blocks to an identity matrix or an equivalent representation. This initialization ensures that the output of the prefix blocks closely matches the input representation, allowing the transformer to see the input as it would without any prefix blocks.

Copy Pretrained Weights: If you have access to pretrained weights for the single-layer transformers, you can directly copy those weights to initialize the prefix blocks. This approach would preserve the initial representations and maintain the original input intact.

Random Initialization: Alternatively, you can initialize the prefix blocks with random weights. However, it's important to initialize them in a way that does not introduce strong biases or distortions to the input representation. Random initialization may introduce noise, but by keeping the magnitude of the random weights small, you can minimize the impact on the input.

Choosing an initialization method ultimately depends on the specifics of your model and the nature of the tasks you are addressing. Initializing the prefix blocks to preserve the input representation ensures that the transformer initially processes the input as it would without any prefix blocks, allowing for a smoother adaptation during fine-tuning.

You can experiment with different initialization approaches and evaluate their impact on the performance of your model to determine which method works best for your specific use case.





User
If I choose to initialize them equivalent to an identity, how would I deal with attention initialization?

ChatGPT
If you choose to initialize the prefix blocks to be equivalent to an identity, you need to handle the attention initialization appropriately. Attention initialization is a crucial step in transformer models as it influences the model's ability to attend to relevant parts of the input.

When initializing the attention mechanism in the prefix blocks to be equivalent to an identity, you can follow these steps:

Mask Attention Weights: To ensure that the attention mechanism starts with an identity-like behavior, you can mask the attention weights during initialization. This prevents the prefix blocks from attending to irrelevant or noisy information initially.

Initialize Positional Embeddings: Positional embeddings play a crucial role in the attention mechanism, allowing the transformer to capture sequential information. When initializing the prefix blocks, you can initialize the positional embeddings to maintain the sequential ordering of the input.

Gradual Unmasking: During the fine-tuning process, you can gradually unmask the attention weights, allowing the prefix blocks to learn task-specific attention patterns. This can be achieved by gradually reducing the masking applied to the attention weights over time.

By masking the attention weights initially and gradually unmasking them during fine-tuning, you allow the prefix blocks to learn task-specific attention patterns while still maintaining some level of initialization that resembles an identity-like behavior.

It's important to note that the specific implementation details may vary depending on the deep learning framework you are using. You may need to refer to the documentation or implementation guidelines of your chosen framework for the precise steps and functions to mask attention weights and initialize positional embeddings.

By carefully handling the attention initialization in the prefix blocks when initializing them to be equivalent to an identity, you can ensure that the model starts with a reasonable attention behavior and gradually adapts to task-specific attention patterns during fine-tuning.





User
I am thinking of actually using LongFormer, both because it can handle longer text without having to discard or split examples in training, but also because of its efficient handling of long attention with the combination of windowed local and global attention.

ChatGPT
Using LongFormer for your model is a great choice, especially if you're dealing with longer texts and want to take advantage of its efficient handling of long attention with windowed local and global attention mechanisms. LongFormer can help maintain contextual information across longer sequences without the need for discarding or splitting examples during training.

When incorporating LongFormer into your model with prefix blocks for different tasks, you can follow these steps:

Define Prefix Blocks: Create four separate prefix blocks, one for each task (MENTION, COREF, ENTITY, RELATION). You can use single-layer LongFormer models as the prefix blocks.

Shared LongFormer Encoder: Use a shared LongFormer encoder for all tasks. This encoder will process the input text and the outputs of the prefix blocks.

Input Encoding: Pass the input text through the shared LongFormer encoder to obtain the input encodings.

Process Prefix Blocks: Feed the input encodings through the respective prefix blocks for each task. Each prefix block will adapt the encodings based on the specific requirements of its task.

Concatenate or Combine Outputs: Depending on the architecture of your model, you can concatenate or combine the outputs of the prefix blocks with the original input encodings. This combination ensures that the original information from the input text is preserved while incorporating the task-specific adaptations from the prefix blocks.

Process Combined Inputs: Pass the combined inputs (original encodings + prefix block outputs) through the shared LongFormer encoder. This allows the model to capture both the task-specific adaptations from the prefix blocks and the contextual information from the input text.

Extract Task-Specific Outputs: After processing the combined inputs through the shared LongFormer encoder, extract the task-specific outputs for each task. These outputs can then be used for further processing or fed into the respective task classifiers.

By incorporating LongFormer into your model architecture and using prefix blocks for each task, you can take advantage of LongFormer's efficient handling of long attention and its ability to handle longer texts without compromising performance.

Remember to freeze the shared LongFormer encoder during training to retain the benefits of pretraining, allowing the model to adapt only through the prefix blocks and the subsequent layers specific to each task.

This approach enables you to leverage LongFormer's capabilities while maintaining task-specific adaptations through the prefix blocks in a multi-task setting.





User
Since we are going to initialize the prefix block in a way equivalent to an identity, and since the prefix block will have its weights adapted, do I really need to combine the original input with the prefix block output?

ChatGPT
Apologies for the confusion in my previous responses. If you initialize the prefix block to be equivalent to an identity and plan to adapt its weights during training, it may not be necessary to combine the original input with the prefix block output.

When the prefix block is initialized as an identity, it means the prefix block initially preserves the original input information and allows the transformer to process the input as if no prefix block were involved. In this case, the prefix block's purpose is to gradually learn task-specific adaptations through weight updates during fine-tuning.

If you don't combine the original input with the prefix block output, the prefix block output alone will be processed by the shared LongFormer encoder. The shared encoder can then capture the task-specific adaptations learned by the prefix block and the contextual information from the input text.

However, please note that the specific design and requirements of your model may vary, and it's important to evaluate the performance and behavior of the model during training and validation. Experimentation and empirical analysis can help determine if combining the original input with the prefix block output improves the model's performance or if using the prefix block output alone is sufficient for your specific task.

Therefore, it is advisable to try both approaches during your experimentation process and choose the option that yields better results in terms of model performance and task-specific objectives.





User
If I don't combine the original input with the prefix block output, and the shared Longformer transformer is frozen, the shared transformer will not adapt its weights, and the only adaptation will be captured by the prefix adaptation.

ChatGPT
You are correct. If you don't combine the original input with the prefix block output and the shared LongFormer transformer is frozen, the adaptation captured by the prefix block will be the primary source of learning and adaptation in your model.

In this case, the prefix block's weights will be updated during training to capture task-specific adaptations, while the weights of the frozen shared LongFormer transformer will remain fixed and preserve the knowledge learned during pretraining.

By omitting the combination of the original input with the prefix block output, you allow the prefix block to directly influence the subsequent layers and task-specific classifiers without interference from the original input.

This approach is known as prefix finetuning, where the frozen transformer is used as a feature extractor, and the prefix block serves as an adaptation module specific to each task. The primary learning and adaptation occur within the prefix block, and the frozen transformer acts as a fixed backbone for feature extraction.

By utilizing prefix finetuning, you can effectively train a multi-task model while avoiding interference and gradient conflicts between the tasks. Each task's objective will guide the adaptation of its respective prefix block, while the shared frozen transformer provides a strong foundation of prelearned representations for all tasks.

Remember to carefully design and validate the performance of your model during training and evaluation to ensure that the prefix block's adaptations capture the necessary task-specific information effectively.





User
Yes, I am trying to use soft prefix finetuning in this case

ChatGPT
Apologies for any confusion caused by my previous responses. If you intend to use soft prefix finetuning, where the prefix block gradually adapts its weights without completely overriding the original input, combining the original input with the prefix block output becomes important.

In soft prefix finetuning, the goal is to allow the prefix block to introduce task-specific adaptations while still preserving the information from the original input. By combining the original input with the prefix block output, you maintain the original information within the model and provide a balanced integration of the task-specific adaptations.

The combination of the original input and the prefix block output can be achieved by concatenating the representations or by any other appropriate merging mechanism. This combined representation is then passed through the frozen shared LongFormer transformer, which acts as a feature extractor, capturing both the contextual information from the original input and the task-specific adaptations introduced by the prefix block.

By incorporating the combined representation into the frozen transformer, you allow the model to benefit from the prelearned representations and capture both the general knowledge learned during pretraining and the task-specific adaptations learned through the prefix block.

It's worth noting that the specific architecture and design choices may depend on the characteristics of your tasks, the available resources, and the nature of the data you're working with. It's recommended to experiment and validate the performance of different approaches to find the most effective configuration for your specific use case.

In summary, soft prefix finetuning with the combination of the original input and the prefix block output allows for a balanced integration of task-specific adaptations while preserving the valuable information from the original input within the model.


2 / 2





User
So let's consider the method by which I should combine the original input to the prefix-adapted output. Since all prefix blocks receive the same input sequence, I will have an output from each prefix block that exactly matches in size. So I could add the input embeddings to the output embeddings. I could also take the mean embeddings. Or I can concatenate the original input to the output of the prefix block, but then I will have a repetition of the same sentence. 
Since I have four tasks, and thus four prefix blocks, and I was planning to use a task dim in the batch to process each of the task prefix outputs separately, I can add a fifth level in the task dimension representing the original input. This will always produce the same output since the tansformer is frozen, and may be wasteful. Also, at the output side of the transformer, I will have to feed some combination of the hidden representation h to the downstream task classifiers. 

ChatGPT
If all the prefix blocks receive the same input sequence and produce output embeddings of the same size, you have a few options to combine the original input with the prefix-adapted output. Here are some approaches to consider:

Addition: You can add the input embeddings to the output embeddings from the prefix block. This approach combines the original information with the task-specific adaptations. The resulting embeddings will have the same dimensionality as the output embeddings.

Mean: Another option is to take the mean of the input embeddings and the output embeddings. This approach can be useful if you want to give equal weight to the original input and the prefix-adapted output.

Concatenation: Instead of directly adding or averaging the embeddings, you can concatenate the original input embeddings with the prefix-adapted output embeddings. This results in a larger combined embedding vector that includes both the original information and the task-specific adaptations. However, as you mentioned, this may introduce redundant repetitions of the same sentence.

Considering the task dimension, adding a fifth level in the task dimension to represent the original input may not be necessary or efficient. Since the transformer is frozen, the original input will produce the same output regardless of the specific task. Instead, you can use the task dimension to process each task's prefix output separately while keeping the original input consistent across all tasks.

At the output side of the transformer, you can extract the hidden representation h and feed it to the downstream task classifiers. Depending on your specific requirements, you can choose to use h as it is or apply further transformations or combinations before passing it to the task classifiers.

In summary, there are multiple ways to combine the original input with the prefix-adapted output, including addition, mean, or concatenation. Consider the specific needs of your tasks and experiment with different approaches to determine the most effective combination method.





User
If I use sum to combine the embeddings, it may make sense to initialize the prefix to produce zero-output instead of identity. 

ChatGPT
If you plan to use the sum operation to combine the embeddings of the original input and the prefix-adapted output, initializing the prefix to produce a zero-output can indeed be a reasonable choice.

By initializing the prefix to produce zero-output, the contribution of the prefix-adapted output to the combined embeddings will be zero initially. This initialization ensures that the original input has a greater influence on the combined representation at the beginning of training.

As training progresses, the prefix block will gradually adapt its weights, and the contribution of the prefix-adapted output will increase. The sum operation will then capture both the original input and the learned task-specific adaptations.

This initialization strategy can be beneficial if you want to prioritize the original input information and allow the prefix block to gradually introduce task-specific adaptations during the training process.

Remember to evaluate the performance of the model during training and validation to ensure that the prefix block is effectively capturing the necessary task-specific information while preserving the valuable information from the original input.

Overall, initializing the prefix to produce zero-output when using the sum operation for combining embeddings can be a suitable approach, as it allows for a controlled integration of the original input and the task-specific adaptations throughout the training process.





User
What would be a suitable initialization for each of the components in a longformer-block-based prefix block?

ChatGPT
When initializing the components of a Longformer-based prefix block, there are several suitable initialization options you can consider:

Positional Embeddings: Longformer models typically utilize sinusoidal positional embeddings to encode the position information of tokens. These embeddings are usually initialized based on a fixed pattern. You can initialize the positional embeddings in the prefix block using the same pattern as the frozen shared Longformer encoder.

Token Embeddings: The token embeddings in the prefix block can be initialized randomly or using pretrained word embeddings if available. You can use the same initialization scheme as the frozen shared Longformer encoder or follow standard practices for initializing token embeddings in transformer models.

Attention Weights: The attention weights in the prefix block can be initialized randomly or using a specific initialization scheme. Depending on the attention mechanism used (e.g., self-attention or windowed attention), you can initialize the attention weights to promote initial attention patterns that prioritize local or global dependencies, as desired. For example, in the case of windowed attention, you can initialize the weights to give higher weights to neighboring tokens.

Feed-forward Layers: The feed-forward layers in the prefix block can be initialized using standard practices for initializing feed-forward networks. Common approaches include initializing the weights with a normal distribution or using a specific initialization scheme like Xavier or He initialization.

The specific choice of initialization scheme for each component in the prefix block may vary depending on the characteristics of your task and data. It's advisable to consider any existing initialization schemes used in the frozen shared Longformer encoder and align the initialization of the prefix block with them for consistency.

Experimentation and empirical analysis can also help determine the most suitable initialization scheme for your specific use case and provide insights into the impact of different initialization strategies on model performance.





User
What would be a reasonable choice for each of the components so that initially it yields zero output which will be summed to the input 

ChatGPT
To achieve an initial zero output from the prefix block, you can consider the following initialization choices for each component:

Positional Embeddings: Initialize the positional embeddings in the prefix block to zero vectors. This will ensure that the initial position information added by the prefix block does not introduce any additional bias.

Token Embeddings: Initialize the token embeddings in the prefix block to zero vectors. This will result in zero contribution from the token embeddings to the initial output of the prefix block.

Attention Weights: Initialize the attention weights in the prefix block to small values, such as small positive or negative numbers close to zero. This initialization can help avoid any strong attention biases initially and allow the model to learn the appropriate attention patterns during training.

Feed-forward Layers: Initialize the weights and biases of the feed-forward layers in the prefix block to zero. This will ensure that the initial output of the feed-forward layers is also zero.

By initializing the components of the prefix block as described above, the initial output of the prefix block will be close to zero. This zero output can then be summed with the input embeddings to yield the combined representation where the original input has a larger influence.

Remember to experiment and evaluate the performance of the model during training and validation to ensure that the prefix block is effectively learning task-specific adaptations while preserving the valuable information from the original input.

Additionally, fine-tuning hyperparameters such as learning rate and regularization can also play a role in controlling the adaptation process of the prefix block and achieving the desired balance between the original input and the task-specific adaptations.





User
So to be more accurate in the architecture description, the prefix block is not placed before the transformer, but between the embedding layer and the encoder layers. 

ChatGPT
Apologies for any confusion caused. You are correct that the prefix block is typically inserted between the embedding layer and the encoder layers, rather than before the entire transformer architecture. I apologize for any misunderstanding in the previous responses.

To clarify the architecture description, the prefix block is added after the input embeddings and before the encoder layers of the transformer model. The prefix block receives the input embeddings, performs its own adaptations (such as additional layers, activations, or attention mechanisms), and then passes the modified representations to the encoder layers for further processing.

The modified representations from the prefix block are then combined with the original input embeddings and processed through the encoder layers of the transformer. This allows the model to leverage both the original input information and the task-specific adaptations introduced by the prefix block during the encoding process.

Once again, I apologize for any confusion caused by the previous responses, and I appreciate your clarification.





User
What is the default value for parameter "add_pooling_layer" in AutoModel.from_config?

ChatGPT
The add_pooling_layer parameter in AutoModel.from_config does not have a default value. When creating an instance of a model using AutoModel.from_config, you need to explicitly specify the value for add_pooling_layer based on your requirements.

The add_pooling_layer parameter is used to determine whether to add a pooling layer on top of the model's encoder output. The pooling layer is typically used to aggregate the contextualized representations into a fixed-length vector, often used for tasks like text classification or sentence-level embeddings.

To specify the value for add_pooling_layer, you can pass it as an argument when calling AutoModel.from_config, for example:

python
Copy code
from transformers import AutoModel

model = AutoModel.from_config(config, add_pooling_layer=True)
In the above example, add_pooling_layer is set to True to indicate that a pooling layer should be added on top of the encoder output. If you want to omit the pooling layer, you can set add_pooling_layer to False.

Please note that the default behavior may vary depending on the specific model configuration and implementation. It's always a good practice to consult the documentation or the source code of the specific model you are using to confirm the default behavior of the add_pooling_layer parameter.





User
what happens if add_pooling_layer is not specified?

ChatGPT
If the add_pooling_layer parameter is not specified when calling AutoModel.from_config, the behavior will depend on the specific implementation and default behavior of the model you are using.

In some implementations, if add_pooling_layer is not specified, the default behavior may be to add a pooling layer on top of the encoder output. This default behavior is often used when the model is commonly applied to tasks that require sentence-level representations or when sentence-level embeddings are commonly used.

However, it's important to note that the default behavior may vary depending on the specific model and implementation. To ensure the desired behavior, it's recommended to consult the documentation or the source code of the specific model you are using to confirm the default behavior when add_pooling_layer is not explicitly specified.

If you want to have more control over whether or not a pooling layer is added, it's recommended to explicitly set the value for add_pooling_layer when calling AutoModel.from_config, either as True or False, based on your specific requirements.





User
In implementing this solution I plan to freeze all layers of the transformer, including the embedding layer which is placed before the prefix block. The prefix block will of course be unfrozen

ChatGPT
If you plan to freeze all layers of the transformer, including the embedding layer that precedes the prefix block, it means that the weights and parameters of those layers will not be updated during training. Only the prefix block, which is unfrozen, will be updated to adapt to the specific task.

In this case, freezing the embedding layer means that the initial word embeddings (e.g., word2vec or GloVe embeddings) or any other pretrained embeddings used in the transformer will remain fixed. The purpose of freezing the transformer layers is to prevent any further updates to the pretrained weights, allowing them to retain the knowledge learned during pretraining.

By keeping the prefix block unfrozen, it can learn task-specific adaptations and contribute to the model's performance on the target task. The prefix block's parameters, including any additional layers, activations, or attention mechanisms, will be updated during training to fine-tune the model for the specific task.

Overall, freezing the transformer layers while keeping the prefix block unfrozen is a common approach to leverage the pretrained knowledge and adapt it to a specific task efficiently. It allows the model to benefit from the general language understanding encoded in the pretrained transformer while enabling task-specific adaptation through the unfrozen prefix block.





User
Currently I call the transformer passing the input of embedding token indexes and the attention_mask to the transformer whose input layer includes the nn.embedding module that turns these indexes to embedding vectors and then goes through the rest of the layers to output the hidden state. In the new prefix implementation, the embedding token indexes will be fed to the nn embedding module preceding the prefix block, and the embedding module of the transformer has to be skipped. How can I do that?  

ChatGPT
To skip the embedding module of the transformer and use the embedding module preceding the prefix block, you can modify the forward pass of your model to pass the input token indexes through the prefix block and then directly to the rest of the layers, bypassing the transformer's embedding module.

Here's an example of how you can modify the forward pass:

python
Copy code
class MyModel(nn.Module):
    def __init__(self, prefix_block, transformer):
        super(MyModel, self).__init__()
        self.prefix_block = prefix_block
        self.transformer = transformer

    def forward(self, input_ids, attention_mask):
        # Pass input through the prefix block
        prefix_output = self.prefix_block(input_ids)

        # Pass the prefix output directly to the rest of the layers
        hidden_state = self.transformer(prefix_output, attention_mask)

        # Perform any additional processing on the hidden state if needed
        # ...

        return hidden_state
In the example above, prefix_block represents your unfrozen prefix block, and transformer represents the frozen transformer with its embedding module. The forward method takes input_ids (token indexes) and attention_mask as input.

First, the input token indexes input_ids are passed through the prefix block using self.prefix_block(input_ids), which applies the necessary adaptations specific to the task.

The output of the prefix block, prefix_output, is then passed directly to the transformer without going through the embedding module. This bypasses the transformer's embedding layer and allows the model to use the embeddings produced by the prefix block.

The rest of the forward pass continues as usual, passing the prefix_output and attention_mask to the transformer's layers and returning the final hidden state.

By modifying the forward pass in this way, you ensure that the input token indexes are processed by the prefix block, and the resulting embeddings are used as input to the transformer, skipping the transformer's own embedding module.





User
what would the self.transformer call look like if I were passing the token IDs instead of embeddings?

ChatGPT
If you want to pass token IDs directly to the transformer instead of embeddings, you can modify the forward pass as follows:

python
Copy code
class MyModel(nn.Module):
    def __init__(self, prefix_block, transformer):
        super(MyModel, self).__init__()
        self.prefix_block = prefix_block
        self.transformer = transformer

    def forward(self, input_ids, attention_mask):
        # Pass input through the prefix block
        prefix_output = self.prefix_block(input_ids)

        # Pass the input_ids directly to the transformer
        hidden_state = self.transformer(input_ids=input_ids, attention_mask=attention_mask)

        # Perform any additional processing on the hidden state if needed
        # ...

        return hidden_state
In this modified version, the input_ids are passed directly to the transformer as input_ids=input_ids, and the attention_mask is also passed.

Note that when passing the token IDs directly to the transformer, you don't need to explicitly provide the embeddings. The transformer model will handle the embedding lookup internally based on the pre-trained embedding weights.

By making this change, you can skip the prefix block's embedding module and pass the raw token IDs to the transformer for further processing.





User
How does the trasnformer know whether it is receiving token-ids or embeddings?

ChatGPT
The transformer model itself does not have inherent knowledge of whether it is receiving token IDs or embeddings. It operates on numerical input representations, which are typically token IDs.

In most transformer-based models, there is an embedding layer at the beginning of the model that maps the token IDs to corresponding embeddings. This embedding layer is responsible for converting the token IDs into dense vector representations (embeddings). The transformer then operates on these embeddings to perform various computations, such as self-attention and feed-forward layers.

The embedding layer is typically a part of the overall model architecture and is trained alongside the other layers. During training, the embedding layer learns to map the token IDs to meaningful embeddings that capture the semantic information of the input tokens. The specific values of the embeddings are updated and learned during the training process.

When passing input to the transformer, you need to ensure that the input is in the form of token IDs (e.g., integer values representing tokens) rather than pre-computed embeddings. The transformer will then internally use its embedding layer to convert the token IDs into corresponding embeddings, which are then processed by the transformer's layers.

Therefore, it is important to use token IDs as input to the transformer and let the model handle the embedding lookup internally. This ensures consistency with the training process and allows the transformer to properly process the input and perform the necessary computations.





User
I suppose when the input is an embedding tensor I should use inputs_embeds argument and if I am feeding token-Ids I should use argument input_ids

ChatGPT
Yes, you're correct. When working with transformers, the choice of using either the inputs_embeds or input_ids argument depends on whether you are directly providing the embedding tensor or the token IDs as input.

Here's a brief explanation of each argument:

inputs_embeds: This argument is used when you already have the precomputed embeddings for your tokens and want to pass them directly to the transformer model. The shape of the inputs_embeds tensor should be (batch_size, sequence_length, embedding_size), where batch_size is the number of input examples, sequence_length is the length of each input sequence, and embedding_size is the dimensionality of the embedding.

input_ids: This argument is used when you have token IDs and want the transformer model to internally perform the embedding lookup. The input_ids tensor should be a tensor of shape (batch_size, sequence_length) where each element represents the integer ID of a token in the vocabulary.

So, depending on whether you have the precomputed embeddings or the token IDs, you should choose the appropriate argument. If you have the token IDs, you can use the input_ids argument, and if you have the embeddings, you can use the inputs_embeds argument.

It's important to note that using the input_ids argument with token IDs will ensure that the transformer model internally performs the embedding lookup using its own embedding layer, which is typically learned during training.





User
I want to use a copy of the transformer's shared embedding layer, which is frozen, to generate the embedding vectors that will be fed to each of the prefix blocks, one for each task. The prefix blocks are single-layer encoder instances of the same transformer type, initialized to output the identity, and later adapted through backpropagation to capture the nuances of each task. The output of the four prefix blocks will be stacked into a minibatch discriminated by an added dimension and passed through the frozen 12-layer transformer. On the output side of the transformer, the four different hidden states will be split and fed to the respective task modules. 

ChatGPT
Based on your description, it seems like you have a clear plan in mind for your model architecture and how you want to utilize the prefix blocks and the shared transformer. Here's a summary of the steps involved:

You have a shared embedding layer within the transformer, which is frozen. This embedding layer maps token IDs to embedding vectors.

You create separate instances of the prefix blocks for each task. Each prefix block is a single-layer encoder of the same transformer type. These prefix blocks are initialized to output the identity.

The input token IDs are passed through the shared embedding layer to obtain the embedding vectors.

The embedding vectors are then fed into each respective prefix block for each task. Each prefix block will process the input embeddings independently.

The output embeddings from each prefix block are stacked into a minibatch, with an additional dimension to discriminate between the tasks.

The stacked embeddings are passed through the frozen 12-layer transformer, which performs its usual computations, including self-attention and feed-forward layers.

On the output side of the transformer, the hidden states corresponding to each task are split, and each hidden state is fed to the respective task module for further processing.

It's important to note that freezing the shared embedding layer ensures that its weights are not updated during training. The prefix blocks, being separate instances, will adapt their weights to capture the task-specific information through backpropagation.

Overall, your approach seems reasonable, and it follows the general idea of using prefix blocks and a shared transformer while adapting the prefix blocks to specific tasks.





User
How can I detach the embedding layer of the transformer and use it before the prefix block?

ChatGPT
To detach the embedding layer of the transformer and use it separately before the prefix block, you can follow these steps:

Create a separate instance of the embedding layer from the transformer. This can be done by accessing the embedding layer from the transformer model and initializing a new instance with the same configuration.

Freeze the parameters of the detached embedding layer to ensure they are not updated during training. This can be achieved by setting the requires_grad attribute of the embedding layer's parameters to False.

Pass your input token IDs through the detached embedding layer to obtain the corresponding embedding vectors. You can use the forward method of the embedding layer to perform this operation.

Feed the embedding vectors to the prefix block for each task, as you described in your architecture. The prefix block will process the embeddings and adapt its weights through backpropagation during training.

Here's an example code snippet to illustrate these steps:

python
Copy code
import torch
import torch.nn as nn
from transformers import AutoModel

# Load the transformer model
model_name = 'bert-base-uncased'
transformer = AutoModel.from_pretrained(model_name)

# Detach the embedding layer from the transformer
embedding_layer = transformer.embeddings
embedding_layer.requires_grad_(False)

# Example input token IDs
input_ids = torch.tensor([[1, 2, 3, 4]])

# Pass input through the detached embedding layer
embeddings = embedding_layer(input_ids)

# Pass the embeddings to the prefix block for each task
prefix_mention = PrefixBlock()
prefix_coref = PrefixBlock()
prefix_entity = PrefixBlock()
prefix_relation = PrefixBlock()

output_mention = prefix_mention(embeddings)
output_coref = prefix_coref(embeddings)
output_entity = prefix_entity(embeddings)
output_relation = prefix_relation(embeddings)

# Continue with the rest of your architecture
# ...
By detaching the embedding layer, you can use it separately before the prefix block while ensuring that its parameters remain fixed.





User
Would it be appropriate to add a statement like:

prefix_mention = copy.deepcopy(transformer.layer[0])
torch.initialize...(prefix_mention)
prefix_coref       = copy.deepcopy(transformer.layer[0])
torch.initialize(prefix_coref)
... etc. for all four prefix blocks?

ChatGPT
Yes, it would be appropriate to use copy.deepcopy() to create separate instances of the prefix blocks based on the first layer of the transformer. This allows you to initialize each prefix block independently and use them in your architecture.

Here's an updated code snippet illustrating the usage of copy.deepcopy() and initialization for each prefix block:

python
Copy code
import torch
import torch.nn as nn
from transformers import AutoModel
import copy

# Load the transformer model
model_name = 'bert-base-uncased'
transformer = AutoModel.from_pretrained(model_name)

# Detach the embedding layer from the transformer
embedding_layer = transformer.embeddings
embedding_layer.requires_grad_(False)

# Example input token IDs
input_ids = torch.tensor([[1, 2, 3, 4]])

# Pass input through the detached embedding layer
embeddings = embedding_layer(input_ids)

# Create separate instances of prefix blocks
prefix_mention = copy.deepcopy(transformer.encoder.layer[0])
prefix_coref = copy.deepcopy(transformer.encoder.layer[0])
prefix_entity = copy.deepcopy(transformer.encoder.layer[0])
prefix_relation = copy.deepcopy(transformer.encoder.layer[0])

# Initialize the prefix blocks
torch.nn.init.xavier_uniform_(prefix_mention.weight)
torch.nn.init.constant_(prefix_mention.bias, 0.0)

torch.nn.init.xavier_uniform_(prefix_coref.weight)
torch.nn.init.constant_(prefix_coref.bias, 0.0)

torch.nn.init.xavier_uniform_(prefix_entity.weight)
torch.nn.init.constant_(prefix_entity.bias, 0.0)

torch.nn.init.xavier_uniform_(prefix_relation.weight)
torch.nn.init.constant_(prefix_relation.bias, 0.0)

# Pass the embeddings to the prefix blocks
output_mention = prefix_mention(embeddings)
output_coref = prefix_coref(embeddings)
output_entity = prefix_entity(embeddings)
output_relation = prefix_relation(embeddings)

# Continue with the rest of your architecture
# ...
Make sure to adjust the indexing transformer.encoder.layer[0] to access the correct layer of the transformer based on your specific transformer model architecture. Additionally, the initialization method used (torch.nn.init.xavier_uniform_) is just an example, and you can choose a different initialization method based on your requirements.





User
I suppose the initialization has to be done for all parameters in the block since the transformer layer contains attention, normalization and output modules within

ChatGPT
Yes, you're correct. When initializing the prefix blocks, you should initialize all the parameters within the block, including the attention, normalization, and output modules.

The initialization should be applied to all relevant parameters within each module in the prefix block. For example, in the case of a transformer layer, you would need to initialize the weights and biases of the self-attention mechanism, the feed-forward neural network, and any other parameters present in the layer.

Here's an updated code snippet that demonstrates the initialization for all parameters within the prefix block:

python
Copy code
import torch
import torch.nn as nn
from transformers import AutoModel
import copy

# Load the transformer model
model_name = 'bert-base-uncased'
transformer = AutoModel.from_pretrained(model_name)

# Detach the embedding layer from the transformer
embedding_layer = transformer.embeddings
embedding_layer.requires_grad_(False)

# Example input token IDs
input_ids = torch.tensor([[1, 2, 3, 4]])

# Pass input through the detached embedding layer
embeddings = embedding_layer(input_ids)

# Create separate instances of prefix blocks
prefix_mention = copy.deepcopy(transformer.encoder.layer[0])
prefix_coref = copy.deepcopy(transformer.encoder.layer[0])
prefix_entity = copy.deepcopy(transformer.encoder.layer[0])
prefix_relation = copy.deepcopy(transformer.encoder.layer[0])

# Initialize the prefix blocks
for module in prefix_mention.modules():
    if isinstance(module, nn.Linear):
        nn.init.xavier_uniform_(module.weight)
        nn.init.constant_(module.bias, 0.0)
    elif isinstance(module, nn.LayerNorm):
        nn.init.constant_(module.weight, 1.0)
        nn.init.constant_(module.bias, 0.0)

for module in prefix_coref.modules():
    # Initialization for prefix_coref modules

for module in prefix_entity.modules():
    # Initialization for prefix_entity modules

for module in prefix_relation.modules():
    # Initialization for prefix_relation modules

# Pass the embeddings to the prefix blocks
output_mention = prefix_mention(embeddings)
output_coref = prefix_coref(embeddings)
output_entity = prefix_entity(embeddings)
output_relation = prefix_relation(embeddings)

# Continue with the rest of your architecture
# ...
Make sure to loop through all the modules within each prefix block and apply the appropriate initialization for each module type.





User
Will this initialization result in zero or close-to-zero output?

ChatGPT
The initialization scheme described in the code snippet I provided does not guarantee zero or close-to-zero output for the prefix blocks. It initializes the weights of the linear layers using Xavier uniform initialization, which aims to set the initial weights such that they are well-suited for the subsequent activation function. The biases are initialized to zero.

The purpose of this initialization is to provide a reasonable starting point for training the prefix blocks. The specific output values after initialization will depend on the specific architecture and the learned parameters of the model.

If you want to ensure zero or close-to-zero output from the prefix blocks, you can modify the initialization scheme accordingly. For example, you could initialize the weights of the linear layers to zeros and biases to zeros as well. This would result in the prefix blocks initially outputting zeros.

Here's an updated code snippet that initializes the linear layers to zeros:

python
Copy code
# Initialize the prefix blocks with zeros
for module in prefix_mention.modules():
    if isinstance(module, nn.Linear):
        nn.init.zeros_(module.weight)
        nn.init.zeros_(module.bias)
    elif isinstance(module, nn.LayerNorm):
        nn.init.constant_(module.weight, 1.0)
        nn.init.constant_(module.bias, 0.0)

# Repeat the initialization for other prefix blocks
# ...
Keep in mind that setting the initial output to exactly zero may not be ideal for training. It could lead to vanishing gradients and hinder the learning process. It's often beneficial to allow the model to start with small random values, such as those provided by Xavier uniform initialization, to introduce some initial diversity in the gradients and enable better learning dynamics.





User
Yes, I think a xavier initialization will prevent multiple paths through the transformer becoming identical. The output of the transformer will eventually be added to the input embeddings and fed to the transformer. How can I make sure that the xavier random perturbations are of minimum magnitude? 

ChatGPT
To ensure that the Xavier random perturbations are of minimum magnitude, you can adjust the gain factor during Xavier initialization. The gain factor determines the scale of the random values added to the weights during initialization.

In PyTorch's nn.init.xavier_uniform_ function, you can specify the gain parameter to control the scale of the initialization. By default, the gain is set to 1.0. Reducing the gain below 1.0 will result in smaller random perturbations.

Here's an example of using a smaller gain value for Xavier initialization:

python
Copy code
import torch.nn as nn

# Initialize the linear layers with Xavier initialization and reduced gain
for module in prefix_mention.modules():
    if isinstance(module, nn.Linear):
        nn.init.xavier_uniform_(module.weight, gain=0.1)
        nn.init.constant_(module.bias, 0.0)

# Repeat the initialization for other prefix blocks
# ...
In the example above, gain=0.1 is used to reduce the magnitude of the random perturbations. You can experiment with different gain values to find the desired level of perturbation for your specific task and model.

Keep in mind that reducing the gain too much may lead to very small weights that can slow down learning or cause vanishing gradients. It's important to strike a balance between introducing sufficient diversity and avoiding extremely small weights that hinder the learning process.





User
will this small perturbation be OK with the frozen pre-trained transformer?

ChatGPT
Yes, introducing small random perturbations through Xavier initialization should generally be fine with a frozen pre-trained transformer. Since the transformer is frozen, its pre-trained weights are not updated during training, and the small perturbations introduced by Xavier initialization will mainly affect the prefix blocks.

The purpose of the small perturbations is to provide some initial diversity in the weights of the prefix blocks, allowing them to capture task-specific information and adapt to the downstream tasks. These perturbations help break the symmetry and ensure that the prefix blocks don't all converge to the same solution.

Since the pre-trained transformer weights are frozen, the small perturbations introduced in the prefix blocks won't significantly impact the learned representations of the transformer layers. The pre-trained weights are already well-optimized for the original pre-training objectives, and the prefix blocks will primarily focus on adapting the model to the specific downstream tasks.

In summary, introducing small perturbations through Xavier initialization is a common practice in transfer learning and fine-tuning scenarios, and it should not negatively impact the frozen pre-trained transformer. It allows the prefix blocks to learn task-specific information while leveraging the knowledge encoded in the pre-trained weights of the transformer layers.

==> X01_data_imbalance_articles.tex <==

Data Imbalance

Dice Loss for Data-imbalanced NLP Tasks (2020) \cite{li-etal-2020-dice} 
(1) the training-test discrepancy (2) the overwhelming effect of easy-negative examples

Focal Loss for Dense Object Detection (2017-2018) \cite{Lin2020FocalLF} 

Distribution-Balanced Loss for Multi-Label Classification in Long-Tailed Datasets \cite{Wu2020DistributionBalancedLF}

Generalized Data Weighting via Class-level Gradient Manipulation 2021 \cite{Chen2021GeneralizedDW} GDW simultaneously mitigates label noise and class imbalance by manipulating gradients at the class level.

Foundations of Data Imbalance (2021) \cite{Kulkarni2021FoundationsOD}

What is the Effect of Importance Weighting in Deep Learning? \cite{Byrd2019WhatIT}
Classification with Noisy Labels by Importance Reweighting \cite{Liu2014ClassificationWN}

Libra R-CNN: Towards Balanced Learning for Object Detection 2019 \cite{Pang2019LibraRT}
three levels - sample level, feature level, and objective level

%===========================================
Multi-Task/Meta-Learning

GradNorm: Gradient Normalization for Adaptive Loss Balancing in Deep Multitask Networks \cite{Chen2018GradNormGN}

Auto-Lambda: Disentangling Dynamic Task Relationships 2022 \cite{Liu2022AutoLambdaDD}

Adapting Auxiliary Losses Using Gradient Similarity 2018 \cite{Du2018AdaptingAL}


==> X90_Cross-EntropyLosses.tex <==

\subsubsection{Cross-Entropy Loss}
This criterion computes the cross entropy loss between input and target.

    It is useful when training a classification problem with $C$ classes.
    If provided, the optional argument ``weight" should be a 1D tensor
    assigning weight to each of the classes.
    This is particularly useful when you have an unbalanced training set.

    The `input` is expected to contain raw, unnormalized scores for each class.
    `input` has to be a Tensor of size $C$ for unbatched input,
    $(minibatch, C)$ or $(minibatch, C, d_1, d_2, ..., d_K)$ with $K \geq 1$ for the
    `K`-dimensional case. The last being useful for higher dimension inputs, such
    as computing cross entropy loss per-pixel for 2D images.

    The `target` that this criterion expects should contain either:

\begin{itemize}
\item     Class indices in the range $[0, C)$ where $C$ is the number of classes; if
      `ignore\_index' is specified, this loss also accepts this class index (this index
      may not necessarily be in the class range). The unreduced (i.e. with attributte `reduction`
      set to `none') loss for this case can be described as:

    \[\ell(x, y) = L = \{l_1,\dots,l_N\}^\top, \quad \]

    where:
    
    \[
    l_n = - w_{y_n} \log \frac{\exp(x_{n,y_n})}{\sum_{c=1}^C \exp(x_{n,c})}
          \cdot \mathbb{1}\{y_n \not= I_{\emptyset}\}        
    \]


      where $x$ is the input, $y$ is the target,
      $I_{\emptyset}$ is the optional ignore-index,
      $w$ is the weight,
      $C$ is the number of classes, and $N$ spans the minibatch dimension. 
        
      Note that this case is equivalent to the combination of :class:`~torch.nn.LogSoftmax` and
      :class:`~torch.nn.NLLLoss`.

\item  Probabilities for each class; useful when labels beyond a single class per minibatch item
      are required, such as for blended labels, label smoothing, etc. The unreduced (i.e. with
      :attr:`reduction` set to `none') loss for this case can be described as:

     \[
          \ell(x, y) = L = \{l_1,\dots,l_N\}^\top, \quad \]

    where:
    \[ l_n = - \sum_{c=1}^C w_c \log \frac{\exp(x_{n,c})}{\sum_{i=1}^C \exp(x_{n,i})} y_{n,c}
    \]
      where $x$ is the input, $y$ is the target, $w$ is the weight,
      $C$ is the number of classes, and $N$ spans the minibatch dimension as well as
      $d_1, ..., d_k$ for the `K`-dimensional case. If
      attribute`reduction' is not `none' (default `mean'), then

 %       \[  \ell(x, y) = \begin{cases} 
 %   \frac{\sum_{n=1}^N l_n}{N} \& \text{if reduction = mean} \\
 %               \sum_{n=1}^N l_n,  \& \text{if reduction} = \text{sum}
 %           \end{cases}
 %   \]

    \end{itemize}

    note:
        The performance of this criterion is generally better when `target` contains class
        indices, as this allows for optimized computation. Consider providing `target` as
        class probabilities only when a single class label per minibatch item is too restrictive.

\subsubsection{BCE-With-Logits Loss}
This loss combines a `Sigmoid` layer and the `BCELoss` in one single
    class. This version is more numerically stable than using a plain `Sigmoid`
    followed by a `BCELoss` as, by combining the operations into one layer,
    we take advantage of the log-sum-exp trick for numerical stability.

    The unreduced (i.e. with :attr:`reduction` set to ``'none'``) loss can be described as:

    \[  \ell(x, y) = L = \{l_1,\dots,l_N\}^\top, \quad \]
    
    where
    
    \[
        l_n = - w_n \left[ y_n \cdot \log \sigma(x_n)
        + (1 - y_n) \cdot \log (1 - \sigma(x_n)) \right]
    \]
    
    with $N$ denoting the batch size. If :attr:`reduction` is not ``'none'``
    (default ``'mean'``), then

    \[
        \ell(x, y) = \begin{cases}
            \overline{L} & \text{if reduction} = \text{mean} \\
            \sum L  &= \text{if reduction} = \text{sum}
        \end{cases}
    \]

    This is used for measuring the error of a reconstruction in for example
    an auto-encoder. Note that the targets `t[i]` should be numbers
    between 0 and 1.

    It's possible to trade off recall and precision by adding weights to positive examples.
    In the case of multi-label classification the loss can be described as:

    \[
        \ell_c(x, y) = L_c = \{l_{1,c},\dots,l_{N,c}\}^\top
    \]
    where 
    \begin{align*}
        l_{n,c} &= - w_{n,c}\, [ p_c y_{n,c} \cdot \log \sigma(x_{n,c}) & \\
        & + (1 - y_{n,c}) \cdot \log (1 - \sigma(x_{n,c})) ]        
    \end{align*}
    
    where $c$ is the class number ($c > 1$) for multi-label binary classification,
    $c = 1$ for single-label binary classification),
    $n$ is the number of the sample in the batch and
    $p_c$ is the weight of the positive answer for the class $c$.

    $p_c > 1$ increases the recall, $p_c < 1$ increases the precision.

    For example, if a dataset contains 100 positive and 300 negative examples of a single class,
    then `pos\_weight` for the class should be equal to $\frac{300}{100}=3$.
    The loss would act as if the dataset contains $3\times 100=300$ positive examples.
    

==> backup/10B-Introduction.tex <==


In this paper, we introduce an innovative Hyperparameter Optimization (HPO) methodology framework for complex machine learning models. Our approach revolves around the concept of 'sprints,' which are individual mini-sessions of hyperparameter exploration and refinement. Each sprint is a focused endeavor, utilizing a specific subset of data and model configuration to optimize hyperparameters effectively.

We formalize our methodology with the introduction of several key concepts:

\begin{description}

\item[Multi-Fidelity Data Splitting:] Each sprint's fidelity is characterized by the fractions of its training and validation data $T/k_T$ and $V/k_V$, named by the two denominators. The identifier ``T6\_V4", indicates that one \nth{6}
 of the training set and one \nth{4} of the validation set is used. This granular approach allows us to finely tune the model with varying data scopes. Multi-fidelity techniques were introduced in conjunction with Hyperband \citep{}  

\item[Model and Parameter Grouping Nomenclature:] Collections of sprints are organized into HPO threads. We distinguish and name these threads by the abbreviated model name, the parameter grouping, and the initialization checkpoint. For example, a thread might be identified as JointMRC-Bert\_GR1\_E13\_S42742, indicating a specific setup of the Joint Multi-Instance Relation Classification model using Bert with a particular parameter grouping (GR1) initialized from a specific checkpoint. Parameter groupings allow for different ways of partitioning model parameters for a more granular association of learning rate or other hyperparameter values. 

\item[Initialization State Identification:] We optimize hyperparameters for different threads of the same model, at different points in the model's training trajectory. The initialization state is denoted by epoch and global step indicators. For example, we use ``E0\_S0" for initializing our model with pre-trained parameters or ``E13\_S42742" for a model initialized from a specific checkpoint taken at epoch 13 and global step 42742. This precise identification ensures clarity and helps us distinguish HPO results whose objective function is initialized at different stages of model finetuning. 

Sprints within a thread can relate in several ways:
\begin{enumerate}[label=(\alph*)]
    \item Replace or Extend: Sprints can either replace a previous sprint or extend it by running additional iterations, thereby building upon previous results.

\item Adjust Dimensions: Subsequent sprints may alter the hyperparameter space, either by pruning unproductive dimensions or expanding them. This is achieved based on prior sprint outcomes, by action invoked by a human in the loop, allowing for a more targeted exploration in subsequent iterations.

\end{enumerate}

\end{description}

When sprints of the same fidelity are extended while adjusting dimensions, we retain the relevant data points from previous sprints that fit within the new boundaries and discard those that fall outside the new boundaries, ensuring continuity and efficiency in our optimization process.

Additionally, our framework supports elevating sprints to higher multi-fidelity levels in two distinct ways. The first approach, which we advocate, involves simply sharing the dimension space of a previous sprint, adjusted if necessary, while disregarding any collected data, effectively starting anew with a higher fidelity but within narrower hyperparameter space boundaries. The second approach capitalizes on the accumulated knowledge by utilizing the hyperparameter combinations (x-values) from previous sprints as starting inputs in the new, more data-intensive sprint. In this latter method, the corresponding performance metrics (y-values) are recalculated using the new surrogate Gaussian Process model, ensuring alignment with the new sprint's Gaussian multivariate distribution. Both approaches offer flexibility in escalating the fidelity (granularity) of the optimized model.

This structured, iterative approach to HPO, encompassing sprints, threading, and multi-fidelity exploration, offers a nuanced and effective strategy for optimizing complex machine learning models. It allows for a detailed and adaptable optimization process, enhancing model performance and efficiency. 



==> compPosMtsAsl.tex <==
\begin{tabular}{lllrrrr}
\toprule
 &  &  & \multicolumn{4}{c}{\textbf{rel-nec-F1-micro}} \\
 &  &  & \textbf{mean} & \textbf{std} & \textbf{min} & \textbf{max} \\
\textbf{POS} & \textbf{MTL} & \textbf{ASL}&  &  &  &  \\
\cmidrule(r){1-7}
\multirow[c]{4}{*}{False} & \multirow[c]{2}{*}{False} & False & 41.73 & 0.40 & 41.21 & 42.10  \\
 &  & True & 41.71 & 0.60 & 40.76 & 42.27 \\
 \cmidrule(r){2-7}
 & \multirow[c]{2}{*}{True} & False & 42.30 & 0.72 & 41.48 & 43.34 \\
 &  & True & 41.72 & 0.78 & 40.49 & 42.40  \\
\cmidrule(r){1-7}
\multirow[c]{4}{*}{True} & \multirow[c]{2}{*}{False} & False & 42.26 & 0.67 & 41.41 & 43.29  \\
 &  & True & 41.55 & 0.44 & 40.97 & 42.05  \\
%\cline{2-7}
\cmidrule(r){2-7}
 & \multirow[c]{2}{*}{True} & False & 42.05 & 0.55 & 41.49 & 42.68  \\
 &  & True & 41.64 & 0.93 & 40.38 & 42.53  \\
 \bottomrule
\end{tabular}

